Cross-temporal probabilistic forecast reconciliation: Methodological and practical issues

Forecast reconciliation is a post-forecasting process that involves transforming a set of incoherent forecasts into coherent forecasts which satisfy a given set of linear constraints for a multivariate time series. In this paper we extend the current state-of-the-art cross-sectional probabilistic forecast reconciliation approach to encompass a cross-temporal framework, where temporal constraints are also applied. Our proposed methodology employs both parametric Gaussian and non-parametric bootstrap approaches to draw samples from an incoherent cross-temporal distribution. To improve the estimation of the forecast error covariance matrix, we propose using multi-step residuals, especially in the time dimension where the usual one-step residuals fail. To address high-dimensionality issues, we present four alternatives for the covariance matrix, where we exploit the two-fold nature (cross-sectional and temporal) of the cross-temporal structure, and introduce the idea of overlapping residuals. We assess the effectiveness of the proposed cross-temporal reconciliation approaches through a simulation study that investigates their theoretical and empirical properties and two forecasting experiments, using the Australian GDP and the Australian Tourism Demand datasets. For both applications, the optimal cross-temporal reconciliation approaches significantly outperform the incoherent base forecasts in terms of the Continuous Ranked Probability Score and the Energy Score. Overall, the results highlight the potential of the proposed methods to improve the accuracy of probabilistic forecasts and to address the challenge of integrating disparate scenarios while coherently taking into account short-term operational, medium-term tactical, and long-term strategic planning.

==> tab/AusGDP/sam_crps.tex <==

\begin{tabular}[t]{l|>{}cccc>{}c|ccccc}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{10}{c}{\textbf{Generation of the base forecasts sample paths}} \\
\cmidrule(l{0pt}r{0pt}){2-11}
\multicolumn{1}{c}{\makecell[c]{\bfseries Reconciliation\\\bfseries approach}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} \\
\multicolumn{1}{c}{} &  & G$_{h}$ & H$_{h}$ & G$_{oh}$ & \multicolumn{1}{c}{H$_{oh}$} &  & G$_{h}$ & H$_{h}$ & G$_{oh}$ & \multicolumn{1}{c}{H$_{oh}$}\\
\midrule
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$\forall k \in \{4,2,1\}$}} & \multicolumn{5}{c}{\textbf{$k = 1$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.979} & \textcolor{black}{0.995} & \textcolor{black}{0.968} & \textcolor{black}{0.976} & \textcolor{black}{1.000} & \textcolor{black}{0.988} & \textcolor{black}{0.988} & \textcolor{black}{0.971} & \textcolor{black}{0.971}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{black}{0.937} & \textcolor{black}{0.956} & \textcolor{black}{0.956} & \textcolor{black}{0.976} & \textcolor{black}{0.976} & \textcolor{black}{0.992} & \textcolor{red}{1.008} & \textcolor{red}{1.008} & \textcolor{red}{1.029} & \textcolor{red}{1.029}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{black}{0.930} & \textcolor{black}{0.917} & \textcolor{black}{0.917} & \textcolor{black}{0.898} & \textcolor{black}{0.898} & \textcolor{black}{0.986} & \textcolor{black}{0.974} & \textcolor{black}{0.975} & \textcolor{black}{0.956} & \textcolor{black}{0.956}\\
oct$_o(wlsv)$ & \textcolor{black}{\textbf{0.926}} & \textcolor{black}{\textbf{0.911}} & \textcolor{black}{\textbf{0.912}} & \textcolor{black}{\textbf{0.896}} & \textcolor{blue}{\textbf{0.895}} & \textcolor{black}{\textbf{0.984}} & \textcolor{black}{\textbf{0.971}} & \textcolor{black}{\textbf{0.970}} & \textcolor{black}{\textbf{0.954}} & \textcolor{blue}{\textbf{0.954}}\\
oct$_o(bdshr)$ & \textcolor{black}{0.978} & \textcolor{black}{0.964} & \textcolor{black}{0.946} & \textcolor{black}{0.952} & \textcolor{black}{0.930} & \textcolor{red}{1.034} & \textcolor{red}{1.016} & \textcolor{red}{1.003} & \textcolor{red}{1.005} & \textcolor{black}{0.989}\\
oct$_{oh}(shr)$ & \textcolor{red}{1.102} & \textcolor{red}{1.059} & \textcolor{red}{1.001} & \textcolor{red}{1.094} & \textcolor{black}{0.988} & \textcolor{red}{1.172} & \textcolor{red}{1.109} & \textcolor{red}{1.066} & \textcolor{red}{1.160} & \textcolor{red}{1.059}\\
oct$_{oh}(hshr)$ & \textcolor{red}{1.006} & \textcolor{black}{0.983} & \textcolor{red}{1.009} & \textcolor{black}{0.974} & \textcolor{red}{1.001} & \textcolor{red}{1.068} & \textcolor{red}{1.046} & \textcolor{red}{1.059} & \textcolor{red}{1.034} & \textcolor{red}{1.061}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 2$}} & \multicolumn{5}{c}{\textbf{$k = 4$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.984} & \textcolor{black}{0.993} & \textcolor{black}{0.968} & \textcolor{black}{0.976} & \textcolor{black}{1.000} & \textcolor{black}{0.966} & \textcolor{red}{1.004} & \textcolor{black}{0.964} & \textcolor{black}{0.981}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{black}{0.949} & \textcolor{black}{0.966} & \textcolor{black}{0.966} & \textcolor{black}{0.987} & \textcolor{black}{0.987} & \textcolor{black}{0.874} & \textcolor{black}{0.896} & \textcolor{black}{0.896} & \textcolor{black}{0.914} & \textcolor{black}{0.914}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{black}{0.942} & \textcolor{black}{0.928} & \textcolor{black}{0.928} & \textcolor{black}{0.909} & \textcolor{black}{0.909} & \textcolor{black}{0.866} & \textcolor{black}{0.853} & \textcolor{black}{0.853} & \textcolor{black}{0.834} & \textcolor{black}{0.834}\\
oct$_o(wlsv)$ & \textcolor{black}{\textbf{0.938}} & \textcolor{black}{\textbf{0.921}} & \textcolor{black}{\textbf{0.923}} & \textcolor{black}{\textbf{0.907}} & \textcolor{blue}{\textbf{0.906}} & \textcolor{black}{\textbf{0.860}} & \textcolor{black}{\textbf{0.847}} & \textcolor{black}{\textbf{0.848}} & \textcolor{black}{\textbf{0.832}} & \textcolor{blue}{\textbf{0.830}}\\
oct$_o(bdshr)$ & \textcolor{black}{0.991} & \textcolor{black}{0.974} & \textcolor{black}{0.957} & \textcolor{black}{0.964} & \textcolor{black}{0.942} & \textcolor{black}{0.914} & \textcolor{black}{0.905} & \textcolor{black}{0.883} & \textcolor{black}{0.892} & \textcolor{black}{0.865}\\
oct$_{oh}(shr)$ & \textcolor{red}{1.120} & \textcolor{red}{1.069} & \textcolor{red}{1.013} & \textcolor{red}{1.113} & \textcolor{red}{1.002} & \textcolor{red}{1.020} & \textcolor{red}{1.002} & \textcolor{black}{0.928} & \textcolor{red}{1.015} & \textcolor{black}{0.909}\\
oct$_{oh}(hshr)$ & \textcolor{red}{1.021} & \textcolor{black}{0.996} & \textcolor{red}{1.021} & \textcolor{black}{0.987} & \textcolor{red}{1.016} & \textcolor{black}{0.934} & \textcolor{black}{0.912} & \textcolor{black}{0.951} & \textcolor{black}{0.904} & \textcolor{black}{0.931}\\
\bottomrule
\multicolumn{11}{l}{\rule{0pt}{1em}\rule{0pt}{1.75em}\makecell[l]{$^\ast$The Gaussian method employs a sample covariance matrix:\\G$_{h}$ and H$_{h}$ use multi-step residuals and G$_{oh}$ and H$_{oh}$ use overlapping and multi-step residuals.}}\\
\end{tabular}


==> tab/AusGDP/sam_es.tex <==

\begin{tabular}[t]{l|>{}cccc>{}c|ccccc}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{10}{c}{\textbf{Generation of the base forecasts sample paths}} \\
\cmidrule(l{0pt}r{0pt}){2-11}
\multicolumn{1}{c}{\makecell[c]{\bfseries Reconciliation\\\bfseries approach}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} \\
\multicolumn{1}{c}{} &  & G$_{h}$ & H$_{h}$ & G$_{oh}$ & \multicolumn{1}{c}{H$_{oh}$} &  & G$_{h}$ & H$_{h}$ & G$_{oh}$ & \multicolumn{1}{c}{H$_{oh}$}\\
\midrule
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$\forall k \in \{4,2,1\}$}} & \multicolumn{5}{c}{\textbf{$k = 1$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.970} & \textcolor{black}{0.988} & \textcolor{black}{0.960} & \textcolor{black}{0.970} & \textcolor{black}{1.000} & \textcolor{black}{0.977} & \textcolor{black}{0.977} & \textcolor{black}{0.965} & \textcolor{black}{0.965}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{black}{0.897} & \textcolor{black}{0.944} & \textcolor{black}{0.944} & \textcolor{black}{0.973} & \textcolor{black}{0.973} & \textcolor{black}{0.964} & \textcolor{red}{1.001} & \textcolor{red}{1.001} & \textcolor{red}{1.033} & \textcolor{red}{1.033}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{black}{\textbf{0.886}} & \textcolor{black}{0.880} & \textcolor{black}{\textbf{0.880}} & \textcolor{blue}{\textbf{0.860}} & \textcolor{black}{\textbf{0.860}} & \textcolor{black}{\textbf{0.954}} & \textcolor{black}{\textbf{0.944}} & \textcolor{black}{\textbf{0.945}} & \textcolor{blue}{\textbf{0.928}} & \textcolor{black}{\textbf{0.928}}\\
oct$_o(wlsv)$ & \textcolor{black}{0.891} & \textcolor{black}{\textbf{0.879}} & \textcolor{black}{0.881} & \textcolor{black}{0.864} & \textcolor{black}{0.864} & \textcolor{black}{0.958} & \textcolor{black}{0.945} & \textcolor{black}{0.945} & \textcolor{black}{0.931} & \textcolor{black}{0.931}\\
oct$_o(bdshr)$ & \textcolor{black}{0.940} & \textcolor{black}{0.928} & \textcolor{black}{0.910} & \textcolor{black}{0.918} & \textcolor{black}{0.895} & \textcolor{red}{1.004} & \textcolor{black}{0.986} & \textcolor{black}{0.971} & \textcolor{black}{0.980} & \textcolor{black}{0.961}\\
oct$_{oh}(shr)$ & \textcolor{red}{1.059} & \textcolor{red}{1.015} & \textcolor{black}{0.956} & \textcolor{red}{1.053} & \textcolor{black}{0.945} & \textcolor{red}{1.130} & \textcolor{red}{1.063} & \textcolor{red}{1.019} & \textcolor{red}{1.121} & \textcolor{red}{1.016}\\
oct$_{oh}(hshr)$ & \textcolor{black}{0.986} & \textcolor{black}{0.968} & \textcolor{black}{0.999} & \textcolor{black}{0.959} & \textcolor{black}{0.992} & \textcolor{red}{1.053} & \textcolor{red}{1.034} & \textcolor{red}{1.049} & \textcolor{red}{1.024} & \textcolor{red}{1.055}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 2$}} & \multicolumn{5}{c}{\textbf{$k = 4$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.972} & \textcolor{black}{0.985} & \textcolor{black}{0.959} & \textcolor{black}{0.969} & \textcolor{black}{1.000} & \textcolor{black}{0.959} & \textcolor{red}{1.000} & \textcolor{black}{0.957} & \textcolor{black}{0.976}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{black}{0.915} & \textcolor{black}{0.961} & \textcolor{black}{0.960} & \textcolor{black}{0.991} & \textcolor{black}{0.991} & \textcolor{black}{0.818} & \textcolor{black}{0.874} & \textcolor{black}{0.874} & \textcolor{black}{0.899} & \textcolor{black}{0.900}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{black}{\textbf{0.904}} & \textcolor{black}{0.896} & \textcolor{black}{\textbf{0.896}} & \textcolor{blue}{\textbf{0.877}} & \textcolor{black}{\textbf{0.877}} & \textcolor{black}{\textbf{0.807}} & \textcolor{black}{0.805} & \textcolor{black}{\textbf{0.805}} & \textcolor{blue}{\textbf{0.782}} & \textcolor{black}{\textbf{0.783}}\\
oct$_o(wlsv)$ & \textcolor{black}{0.908} & \textcolor{black}{\textbf{0.895}} & \textcolor{black}{0.898} & \textcolor{black}{0.881} & \textcolor{black}{0.882} & \textcolor{black}{0.812} & \textcolor{black}{\textbf{0.802}} & \textcolor{black}{0.806} & \textcolor{black}{0.786} & \textcolor{black}{0.786}\\
oct$_o(bdshr)$ & \textcolor{black}{0.960} & \textcolor{black}{0.947} & \textcolor{black}{0.929} & \textcolor{black}{0.938} & \textcolor{black}{0.915} & \textcolor{black}{0.860} & \textcolor{black}{0.856} & \textcolor{black}{0.836} & \textcolor{black}{0.841} & \textcolor{black}{0.816}\\
oct$_{oh}(shr)$ & \textcolor{red}{1.082} & \textcolor{red}{1.029} & \textcolor{black}{0.973} & \textcolor{red}{1.076} & \textcolor{black}{0.963} & \textcolor{black}{0.971} & \textcolor{black}{0.954} & \textcolor{black}{0.882} & \textcolor{black}{0.967} & \textcolor{black}{0.861}\\
oct$_{oh}(hshr)$ & \textcolor{red}{1.007} & \textcolor{black}{0.988} & \textcolor{red}{1.017} & \textcolor{black}{0.979} & \textcolor{red}{1.014} & \textcolor{black}{0.904} & \textcolor{black}{0.888} & \textcolor{black}{0.934} & \textcolor{black}{0.881} & \textcolor{black}{0.913}\\
\bottomrule
\multicolumn{11}{l}{\rule{0pt}{1em}\rule{0pt}{1.75em}\makecell[l]{$^\ast$The Gaussian method employs a sample covariance matrix:\\G$_{h}$ and H$_{h}$ use multi-step residuals and G$_{oh}$ and H$_{oh}$ use overlapping and multi-step residuals.}}\\
\end{tabular}


==> tab/Sim/norm_cov.tex <==

\begin{tabular}[t]{l|>{}ccccc}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{5}{c}{\textbf{Generation of the base forecasts paths}} \\
\cmidrule(l{0pt}r{0pt}){2-6}
\multicolumn{1}{c}{\makecell[c]{\bfseries Reconciliation\\\bfseries approach}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} \\
\multicolumn{1}{c}{} &  & G & B & H & HB\\
\midrule
base & \textcolor{black}{8.260} & \textcolor{black}{7.748} & \textcolor{black}{6.549} & \textcolor{black}{3.409} & \textcolor{black}{2.215}\\
ct$(bu)$ & \textcolor{black}{3.195} & \textcolor{black}{2.215} & \textcolor{black}{2.215} & \textcolor{black}{\textbf{2.215}} & \textcolor{black}{2.215}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{black}{3.202} & \textcolor{black}{2.224} & \textcolor{black}{2.215} & \textcolor{black}{2.224} & \textcolor{black}{2.215}\\
ct$(wlsv_{te}, bu_{cs})$ & \textcolor{black}{\textbf{3.183}} & \textcolor{black}{\textbf{2.188}} & \textcolor{black}{2.188} & \textcolor{black}{\textbf{2.215}} & \textcolor{black}{2.215}\\
oct$(wlsv)$ & \textcolor{black}{3.766} & \textcolor{black}{3.082} & \textcolor{black}{2.191} & \textcolor{black}{2.910} & \textcolor{black}{2.215}\\
oct$(bdshr)$ & \textcolor{black}{3.203} & \textcolor{black}{2.195} & \textcolor{blue}{\textbf{2.184}} & \textcolor{black}{2.224} & \textcolor{black}{\textbf{2.215}}\\
oct$_h(shr)$ & \textcolor{black}{3.251} & \textcolor{black}{2.260} & \textcolor{black}{2.202} & \textcolor{black}{2.226} & \textcolor{black}{2.215}\\
oct$_h(bshr)$ & \textcolor{black}{3.602} & \textcolor{black}{2.720} & \textcolor{black}{2.220} & \textcolor{black}{2.756} & \textcolor{black}{2.215}\\
oct$_h(hshr)$ & \textcolor{black}{4.869} & \textcolor{black}{4.138} & \textcolor{black}{4.167} & \textcolor{black}{2.225} & \textcolor{black}{2.215}\\
oct$_h(hbshr)$ & \textcolor{black}{5.731} & \textcolor{black}{5.085} & \textcolor{black}{4.167} & \textcolor{black}{2.756} & \textcolor{black}{2.215}\\
\bottomrule
\multicolumn{6}{l}{\rule{0pt}{1em}\rule{0pt}{1.75em}\makecell[l]{$^\ast$The Gaussian method employs a sample covariance\\ with multi-step residuals.}}\\
\end{tabular}


==> tab/Sim/sam_crps.tex <==

\begin{tabular}[t]{l|>{}cccc>{}c|ccccc}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{10}{c}{\textbf{Generation of the base forecasts sample paths}} \\
\cmidrule(l{0pt}r{0pt}){2-11}
\multicolumn{1}{c}{\makecell[c]{\bfseries Reconciliation\\\bfseries approach}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} \\
\multicolumn{1}{c}{} &  & G & B & H & \multicolumn{1}{c}{HB} &  & G & B & H & HB\\
\midrule
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$\forall k \in \{2,1\}$}} & \multicolumn{5}{c}{\textbf{$k = 1$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.998} & \textcolor{black}{0.999} & \textcolor{red}{1.002} & \textcolor{red}{1.004} & \textcolor{black}{1.000} & \textcolor{black}{0.998} & \textcolor{black}{0.999} & \textcolor{black}{0.999} & \textcolor{black}{1.000}\\
ct$(bu)$ & \textcolor{black}{0.901} & \textcolor{black}{0.900} & \textcolor{black}{0.900} & \textcolor{black}{0.900} & \textcolor{black}{0.900} & \textcolor{black}{0.978} & \textcolor{black}{0.976} & \textcolor{black}{0.976} & \textcolor{black}{0.977} & \textcolor{black}{0.977}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{black}{\textbf{0.901}} & \textcolor{black}{\textbf{0.900}} & \textcolor{blue}{\textbf{0.899}} & \textcolor{black}{\textbf{0.900}} & \textcolor{black}{\textbf{0.900}} & \textcolor{black}{\textbf{0.977}} & \textcolor{black}{\textbf{0.976}} & \textcolor{blue}{\textbf{0.976}} & \textcolor{black}{\textbf{0.976}} & \textcolor{black}{\textbf{0.976}}\\
ct$(wlsv_{te}, bu_{cs})$ & \textcolor{black}{0.910} & \textcolor{black}{0.916} & \textcolor{black}{0.916} & \textcolor{black}{0.916} & \textcolor{black}{0.917} & \textcolor{black}{0.986} & \textcolor{black}{0.993} & \textcolor{black}{0.993} & \textcolor{black}{0.993} & \textcolor{black}{0.993}\\
oct$(wlsv)$ & \textcolor{black}{0.922} & \textcolor{black}{0.930} & \textcolor{black}{0.930} & \textcolor{black}{0.930} & \textcolor{black}{0.931} & \textcolor{black}{0.998} & \textcolor{red}{1.006} & \textcolor{red}{1.006} & \textcolor{red}{1.007} & \textcolor{red}{1.007}\\
oct$(bdshr)$ & \textcolor{black}{0.910} & \textcolor{black}{0.916} & \textcolor{black}{0.915} & \textcolor{black}{0.916} & \textcolor{black}{0.916} & \textcolor{black}{0.986} & \textcolor{black}{0.992} & \textcolor{black}{0.992} & \textcolor{black}{0.993} & \textcolor{black}{0.993}\\
oct$_h(shr)$ & \textcolor{black}{0.904} & \textcolor{black}{0.903} & \textcolor{black}{0.902} & \textcolor{black}{0.902} & \textcolor{black}{0.903} & \textcolor{black}{0.980} & \textcolor{black}{0.979} & \textcolor{black}{0.978} & \textcolor{black}{0.979} & \textcolor{black}{0.979}\\
oct$_h(bshr)$ & \textcolor{black}{0.923} & \textcolor{black}{0.922} & \textcolor{black}{0.922} & \textcolor{black}{0.921} & \textcolor{black}{0.922} & \textcolor{black}{0.999} & \textcolor{black}{0.998} & \textcolor{black}{0.998} & \textcolor{black}{0.998} & \textcolor{black}{0.998}\\
oct$_h(hshr)$ & \textcolor{black}{0.974} & \textcolor{black}{0.972} & \textcolor{black}{0.972} & \textcolor{black}{0.974} & \textcolor{black}{0.975} & \textcolor{red}{1.052} & \textcolor{red}{1.050} & \textcolor{red}{1.050} & \textcolor{red}{1.053} & \textcolor{red}{1.053}\\
oct$_h(hbshr)$ & \textcolor{black}{0.987} & \textcolor{black}{0.985} & \textcolor{black}{0.985} & \textcolor{black}{0.987} & \textcolor{black}{0.989} & \textcolor{red}{1.065} & \textcolor{red}{1.063} & \textcolor{red}{1.064} & \textcolor{red}{1.066} & \textcolor{red}{1.068}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 2$}} & \multicolumn{5}{c}{}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.998} & \textcolor{black}{0.999} & \textcolor{red}{1.005} & \textcolor{red}{1.008} &  &  &  &  & \\
ct$(bu)$ & \textcolor{black}{0.831} & \textcolor{black}{0.830} & \textcolor{black}{0.829} & \textcolor{black}{0.829} & \textcolor{black}{0.830} &  &  &  &  & \\
ct$(shr_{cs}, bu_{te})$ & \textcolor{black}{\textbf{0.830}} & \textcolor{black}{\textbf{0.830}} & \textcolor{blue}{\textbf{0.829}} & \textcolor{black}{\textbf{0.829}} & \textcolor{black}{\textbf{0.830}} &  &  &  &  & \\
ct$(wlsv_{te}, bu_{cs})$ & \textcolor{black}{0.840} & \textcolor{black}{0.846} & \textcolor{black}{0.844} & \textcolor{black}{0.845} & \textcolor{black}{0.846} &  &  &  &  & \\
oct$(wlsv)$ & \textcolor{black}{0.851} & \textcolor{black}{0.859} & \textcolor{black}{0.859} & \textcolor{black}{0.859} & \textcolor{black}{0.861} &  &  &  &  & \\
oct$(bdshr)$ & \textcolor{black}{0.839} & \textcolor{black}{0.845} & \textcolor{black}{0.844} & \textcolor{black}{0.845} & \textcolor{black}{0.846} &  &  &  &  & \\
oct$_h(shr)$ & \textcolor{black}{0.834} & \textcolor{black}{0.833} & \textcolor{black}{0.831} & \textcolor{black}{0.832} & \textcolor{black}{0.832} &  &  &  &  & \\
oct$_h(bshr)$ & \textcolor{black}{0.852} & \textcolor{black}{0.851} & \textcolor{black}{0.851} & \textcolor{black}{0.851} & \textcolor{black}{0.852} &  &  &  &  & \\
oct$_h(hshr)$ & \textcolor{black}{0.902} & \textcolor{black}{0.900} & \textcolor{black}{0.899} & \textcolor{black}{0.901} & \textcolor{black}{0.902} &  &  &  &  & \\
oct$_h(hbshr)$ & \textcolor{black}{0.915} & \textcolor{black}{0.913} & \textcolor{black}{0.913} & \textcolor{black}{0.914} & \textcolor{black}{0.917} &  &  &  &  & \\
\bottomrule
\multicolumn{11}{l}{\rule{0pt}{1em}\rule{0pt}{1.75em}\makecell[l]{$^\ast$The Gaussian method employs a sample covariance matrix and includes four techniques\\ (G, B, H, HB) with multi-step residuals.}}\\
\end{tabular}


==> tab/Sim/sam_es.tex <==

\begin{tabular}[t]{l|>{}cccc>{}c|ccccc}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{10}{c}{\textbf{Generation of the base forecasts sample paths}} \\
\cmidrule(l{0pt}r{0pt}){2-11}
\multicolumn{1}{c}{\makecell[c]{\bfseries Reconciliation\\\bfseries approach}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} \\
\multicolumn{1}{c}{} &  & G & B & H & \multicolumn{1}{c}{HB} &  & G & B & H & HB\\
\midrule
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$\forall k \in \{2,1\}$}} & \multicolumn{5}{c}{\textbf{$k = 1$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.996} & \textcolor{black}{0.999} & \textcolor{black}{1.000} & \textcolor{red}{1.004} & \textcolor{black}{1.000} & \textcolor{black}{0.997} & \textcolor{red}{1.000} & \textcolor{black}{0.997} & \textcolor{red}{1.000}\\
ct$(bu)$ & \textcolor{black}{0.897} & \textcolor{black}{0.895} & \textcolor{black}{0.896} & \textcolor{black}{0.897} & \textcolor{blue}{\textbf{0.895}} & \textcolor{black}{0.969} & \textcolor{black}{\textbf{0.967}} & \textcolor{blue}{\textbf{0.967}} & \textcolor{black}{0.968} & \textcolor{black}{\textbf{0.968}}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{black}{\textbf{0.896}} & \textcolor{black}{\textbf{0.895}} & \textcolor{black}{\textbf{0.895}} & \textcolor{black}{\textbf{0.896}} & \textcolor{black}{0.896} & \textcolor{black}{\textbf{0.968}} & \textcolor{black}{0.968} & \textcolor{black}{0.967} & \textcolor{black}{\textbf{0.968}} & \textcolor{black}{0.968}\\
ct$(wlsv_{te}, bu_{cs})$ & \textcolor{black}{0.906} & \textcolor{black}{0.912} & \textcolor{black}{0.911} & \textcolor{black}{0.910} & \textcolor{black}{0.912} & \textcolor{black}{0.977} & \textcolor{black}{0.984} & \textcolor{black}{0.983} & \textcolor{black}{0.981} & \textcolor{black}{0.984}\\
oct$(wlsv)$ & \textcolor{black}{0.916} & \textcolor{black}{0.923} & \textcolor{black}{0.923} & \textcolor{black}{0.923} & \textcolor{black}{0.924} & \textcolor{black}{0.989} & \textcolor{black}{0.994} & \textcolor{black}{0.995} & \textcolor{black}{0.995} & \textcolor{black}{0.997}\\
oct$(bdshr)$ & \textcolor{black}{0.906} & \textcolor{black}{0.910} & \textcolor{black}{0.910} & \textcolor{black}{0.911} & \textcolor{black}{0.912} & \textcolor{black}{0.977} & \textcolor{black}{0.981} & \textcolor{black}{0.982} & \textcolor{black}{0.983} & \textcolor{black}{0.985}\\
oct$_h(shr)$ & \textcolor{black}{0.900} & \textcolor{black}{0.898} & \textcolor{black}{0.898} & \textcolor{black}{0.897} & \textcolor{black}{0.898} & \textcolor{black}{0.971} & \textcolor{black}{0.969} & \textcolor{black}{0.969} & \textcolor{black}{0.969} & \textcolor{black}{0.969}\\
oct$_h(bshr)$ & \textcolor{black}{0.916} & \textcolor{black}{0.914} & \textcolor{black}{0.916} & \textcolor{black}{0.915} & \textcolor{black}{0.916} & \textcolor{black}{0.987} & \textcolor{black}{0.986} & \textcolor{black}{0.987} & \textcolor{black}{0.987} & \textcolor{black}{0.988}\\
oct$_h(hshr)$ & \textcolor{black}{0.967} & \textcolor{black}{0.964} & \textcolor{black}{0.964} & \textcolor{black}{0.966} & \textcolor{black}{0.967} & \textcolor{red}{1.040} & \textcolor{red}{1.036} & \textcolor{red}{1.036} & \textcolor{red}{1.040} & \textcolor{red}{1.040}\\
oct$_h(hbshr)$ & \textcolor{black}{0.978} & \textcolor{black}{0.975} & \textcolor{black}{0.976} & \textcolor{black}{0.977} & \textcolor{black}{0.980} & \textcolor{red}{1.051} & \textcolor{red}{1.047} & \textcolor{red}{1.049} & \textcolor{red}{1.051} & \textcolor{red}{1.052}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 2$}} & \multicolumn{5}{c}{}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.996} & \textcolor{black}{0.998} & \textcolor{red}{1.003} & \textcolor{red}{1.008} &  &  &  &  & \\
ct$(bu)$ & \textcolor{black}{0.831} & \textcolor{black}{0.829} & \textcolor{black}{0.829} & \textcolor{black}{0.830} & \textcolor{blue}{\textbf{0.828}} &  &  &  &  & \\
ct$(shr_{cs}, bu_{te})$ & \textcolor{black}{\textbf{0.829}} & \textcolor{black}{\textbf{0.828}} & \textcolor{black}{\textbf{0.829}} & \textcolor{black}{\textbf{0.829}} & \textcolor{black}{0.829} &  &  &  &  & \\
ct$(wlsv_{te}, bu_{cs})$ & \textcolor{black}{0.839} & \textcolor{black}{0.844} & \textcolor{black}{0.844} & \textcolor{black}{0.844} & \textcolor{black}{0.845} &  &  &  &  & \\
oct$(wlsv)$ & \textcolor{black}{0.849} & \textcolor{black}{0.858} & \textcolor{black}{0.856} & \textcolor{black}{0.856} & \textcolor{black}{0.857} &  &  &  &  & \\
oct$(bdshr)$ & \textcolor{black}{0.839} & \textcolor{black}{0.845} & \textcolor{black}{0.843} & \textcolor{black}{0.845} & \textcolor{black}{0.844} &  &  &  &  & \\
oct$_h(shr)$ & \textcolor{black}{0.835} & \textcolor{black}{0.833} & \textcolor{black}{0.833} & \textcolor{black}{0.831} & \textcolor{black}{0.832} &  &  &  &  & \\
oct$_h(bshr)$ & \textcolor{black}{0.850} & \textcolor{black}{0.847} & \textcolor{black}{0.849} & \textcolor{black}{0.849} & \textcolor{black}{0.850} &  &  &  &  & \\
oct$_h(hshr)$ & \textcolor{black}{0.900} & \textcolor{black}{0.897} & \textcolor{black}{0.896} & \textcolor{black}{0.897} & \textcolor{black}{0.899} &  &  &  &  & \\
oct$_h(hbshr)$ & \textcolor{black}{0.910} & \textcolor{black}{0.907} & \textcolor{black}{0.908} & \textcolor{black}{0.909} & \textcolor{black}{0.912} &  &  &  &  & \\
\bottomrule
\multicolumn{11}{l}{\rule{0pt}{1em}\rule{0pt}{1.75em}\makecell[l]{$^\ast$The Gaussian method employs a sample covariance matrix and includes four techniques\\ (G, B, H, HB) with multi-step residuals.}}\\
\end{tabular}


==> tab/VN525/sam_crps_more.tex <==

\begin{tabular}[t]{c|>{}cccc>{}c|ccccc}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{10}{c}{\textbf{Base forecasts' sample approach}} \\
\cmidrule(l{0pt}r{0pt}){2-11}
\multicolumn{1}{c}{\makecell[c]{\bfseries Reconciliation\\\bfseries approach}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} \\
\multicolumn{1}{c}{} &  & G & B & H & \multicolumn{1}{c}{HB} &  & G & B & H & HB\\
\midrule
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$\forall k \in \{12,6,4,3,2,1\}$}} & \multicolumn{5}{c}{\textbf{$k = 1$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.971} & \textcolor{black}{0.971} & \textcolor{black}{0.973} & \textcolor{black}{0.973} & \textcolor{black}{1.000} & \textcolor{black}{0.972} & \textcolor{black}{0.972} & \textcolor{black}{0.972} & \textcolor{black}{0.972}\\
ct$(bu)$ & \textcolor{red}{1.321} & \textcolor{red}{1.011} & \textcolor{red}{1.011} & \textcolor{red}{1.011} & \textcolor{red}{1.011} & \textcolor{red}{1.077} & \textcolor{black}{0.983} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.982}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.057} & \textcolor{black}{0.974} & \textcolor{black}{0.969} & \textcolor{black}{0.974} & \textcolor{black}{0.969} & \textcolor{black}{0.976} & \textcolor{black}{0.963} & \textcolor{black}{0.962} & \textcolor{black}{0.963} & \textcolor{black}{0.962}\\
ct$(wlsv_{te}, bu_{cs})$ & \textcolor{red}{1.062} & \textcolor{black}{0.974} & \textcolor{black}{0.974} & \textcolor{black}{0.972} & \textcolor{black}{0.972} & \textcolor{black}{0.976} & \textcolor{black}{0.965} & \textcolor{black}{0.965} & \textcolor{black}{0.966} & \textcolor{black}{0.966}\\
oct$(ols)$ & \textcolor{black}{0.989} & \textcolor{black}{0.989} & \textcolor{black}{0.989} & \textcolor{black}{0.987} & \textcolor{black}{0.987} & \textcolor{black}{0.982} & \textcolor{black}{0.986} & \textcolor{black}{0.988} & \textcolor{black}{0.986} & \textcolor{black}{0.989}\\
oct$(struc)$ & \textcolor{black}{0.982} & \textcolor{black}{0.962} & \textcolor{black}{0.961} & \textcolor{black}{0.961} & \textcolor{black}{0.959} & \textcolor{black}{0.970} & \textcolor{black}{0.963} & \textcolor{black}{0.963} & \textcolor{black}{0.963} & \textcolor{black}{0.963}\\
oct$(wlsv)$ & \textcolor{black}{0.987} & \textcolor{black}{0.959} & \textcolor{black}{0.959} & \textcolor{black}{0.958} & \textcolor{black}{0.957} & \textcolor{black}{0.952} & \textcolor{black}{0.957} & \textcolor{black}{0.957} & \textcolor{black}{0.957} & \textcolor{black}{0.957}\\
oct$(bdshr)$ & \textcolor{black}{0.975} & \textcolor{black}{\textbf{0.956}} & \textcolor{black}{\textbf{0.953}} & \textcolor{black}{\textbf{0.952}} & \textcolor{blue}{\textbf{0.951}} & \textcolor{blue}{\textbf{0.949}} & \textcolor{black}{\textbf{0.955}} & \textcolor{black}{\textbf{0.953}} & \textcolor{black}{\textbf{0.954}} & \textcolor{black}{\textbf{0.954}}\\
oct$_h(hbshr)$ & \textcolor{black}{0.989} & \textcolor{red}{1.018} & \textcolor{red}{1.020} & \textcolor{red}{1.016} & \textcolor{red}{1.018} & \textcolor{black}{0.982} & \textcolor{red}{1.004} & \textcolor{red}{1.007} & \textcolor{red}{1.004} & \textcolor{red}{1.009}\\
oct$_h(bshr)$ & \textcolor{black}{0.994} & \textcolor{red}{1.018} & \textcolor{red}{1.020} & \textcolor{red}{1.016} & \textcolor{red}{1.019} & \textcolor{black}{0.988} & \textcolor{red}{1.007} & \textcolor{red}{1.013} & \textcolor{red}{1.006} & \textcolor{red}{1.012}\\
oct$_h(hshr)$ & \textcolor{black}{\textbf{0.969}} & \textcolor{black}{0.993} & \textcolor{black}{0.993} & \textcolor{black}{0.990} & \textcolor{black}{0.991} & \textcolor{black}{0.953} & \textcolor{black}{0.977} & \textcolor{black}{0.977} & \textcolor{black}{0.979} & \textcolor{black}{0.979}\\
oct$_h(shr)$ & \textcolor{red}{1.007} & \textcolor{black}{0.980} & \textcolor{black}{0.972} & \textcolor{black}{0.970} & \textcolor{black}{0.970} & \textcolor{red}{1.000} & \textcolor{black}{0.986} & \textcolor{black}{0.977} & \textcolor{black}{0.976} & \textcolor{black}{0.974}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 2$}} & \multicolumn{5}{c}{\textbf{$k = 3$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.970} & \textcolor{black}{0.969} & \textcolor{black}{0.970} & \textcolor{black}{0.971} & \textcolor{black}{1.000} & \textcolor{black}{0.971} & \textcolor{black}{0.971} & \textcolor{black}{0.972} & \textcolor{black}{0.973}\\
ct$(bu)$ & \textcolor{red}{1.189} & \textcolor{black}{0.999} & \textcolor{black}{0.999} & \textcolor{black}{0.999} & \textcolor{black}{0.999} & \textcolor{red}{1.273} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.010}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.015} & \textcolor{black}{0.972} & \textcolor{black}{0.970} & \textcolor{black}{0.972} & \textcolor{black}{0.970} & \textcolor{red}{1.041} & \textcolor{black}{0.977} & \textcolor{black}{0.974} & \textcolor{black}{0.977} & \textcolor{black}{0.974}\\
ct$(wlsv_{te}, bu_{cs})$ & \textcolor{red}{1.016} & \textcolor{black}{0.971} & \textcolor{black}{0.971} & \textcolor{black}{0.970} & \textcolor{black}{0.970} & \textcolor{red}{1.046} & \textcolor{black}{0.976} & \textcolor{black}{0.976} & \textcolor{black}{0.974} & \textcolor{black}{0.974}\\
oct$(ols)$ & \textcolor{black}{0.992} & \textcolor{black}{0.991} & \textcolor{black}{0.991} & \textcolor{black}{0.990} & \textcolor{black}{0.991} & \textcolor{black}{0.994} & \textcolor{black}{0.992} & \textcolor{black}{0.993} & \textcolor{black}{0.991} & \textcolor{black}{0.992}\\
oct$(struc)$ & \textcolor{black}{0.982} & \textcolor{black}{0.966} & \textcolor{black}{0.965} & \textcolor{black}{0.965} & \textcolor{black}{0.965} & \textcolor{black}{0.986} & \textcolor{black}{0.967} & \textcolor{black}{0.966} & \textcolor{black}{0.966} & \textcolor{black}{0.965}\\
oct$(wlsv)$ & \textcolor{black}{0.972} & \textcolor{black}{0.961} & \textcolor{black}{0.960} & \textcolor{black}{0.960} & \textcolor{black}{0.960} & \textcolor{black}{0.983} & \textcolor{black}{0.963} & \textcolor{black}{0.962} & \textcolor{black}{0.962} & \textcolor{black}{0.962}\\
oct$(bdshr)$ & \textcolor{black}{\textbf{0.964}} & \textcolor{black}{\textbf{0.958}} & \textcolor{black}{\textbf{0.957}} & \textcolor{black}{\textbf{0.956}} & \textcolor{blue}{\textbf{0.956}} & \textcolor{black}{0.972} & \textcolor{black}{\textbf{0.960}} & \textcolor{black}{\textbf{0.958}} & \textcolor{black}{\textbf{0.957}} & \textcolor{blue}{\textbf{0.957}}\\
oct$_h(hbshr)$ & \textcolor{black}{0.992} & \textcolor{red}{1.013} & \textcolor{red}{1.015} & \textcolor{red}{1.012} & \textcolor{red}{1.015} & \textcolor{black}{0.994} & \textcolor{red}{1.019} & \textcolor{red}{1.021} & \textcolor{red}{1.018} & \textcolor{red}{1.020}\\
oct$_h(bshr)$ & \textcolor{black}{0.997} & \textcolor{red}{1.015} & \textcolor{red}{1.018} & \textcolor{red}{1.013} & \textcolor{red}{1.017} & \textcolor{black}{0.999} & \textcolor{red}{1.021} & \textcolor{red}{1.022} & \textcolor{red}{1.018} & \textcolor{red}{1.022}\\
oct$_h(hshr)$ & \textcolor{black}{0.965} & \textcolor{black}{0.987} & \textcolor{black}{0.987} & \textcolor{black}{0.986} & \textcolor{black}{0.987} & \textcolor{black}{\textbf{0.971}} & \textcolor{black}{0.994} & \textcolor{black}{0.994} & \textcolor{black}{0.992} & \textcolor{black}{0.993}\\
oct$_h(shr)$ & \textcolor{red}{1.005} & \textcolor{black}{0.986} & \textcolor{black}{0.978} & \textcolor{black}{0.976} & \textcolor{black}{0.975} & \textcolor{red}{1.009} & \textcolor{black}{0.986} & \textcolor{black}{0.978} & \textcolor{black}{0.976} & \textcolor{black}{0.976}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 4$}} & \multicolumn{5}{c}{\textbf{$k = 6$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.973} & \textcolor{black}{0.973} & \textcolor{black}{0.974} & \textcolor{black}{0.975} & \textcolor{black}{1.000} & \textcolor{black}{0.976} & \textcolor{black}{0.976} & \textcolor{black}{0.978} & \textcolor{black}{0.978}\\
ct$(bu)$ & \textcolor{red}{1.340} & \textcolor{red}{1.016} & \textcolor{red}{1.015} & \textcolor{red}{1.015} & \textcolor{red}{1.015} & \textcolor{red}{1.450} & \textcolor{red}{1.023} & \textcolor{red}{1.023} & \textcolor{red}{1.023} & \textcolor{red}{1.023}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.061} & \textcolor{black}{0.978} & \textcolor{black}{0.973} & \textcolor{black}{0.978} & \textcolor{black}{0.973} & \textcolor{red}{1.094} & \textcolor{black}{0.978} & \textcolor{black}{0.972} & \textcolor{black}{0.978} & \textcolor{black}{0.972}\\
ct$(wlsv_{te}, bu_{cs})$ & \textcolor{red}{1.068} & \textcolor{black}{0.977} & \textcolor{black}{0.977} & \textcolor{black}{0.974} & \textcolor{black}{0.974} & \textcolor{red}{1.103} & \textcolor{black}{0.977} & \textcolor{black}{0.977} & \textcolor{black}{0.974} & \textcolor{black}{0.974}\\
oct$(ols)$ & \textcolor{black}{0.993} & \textcolor{black}{0.991} & \textcolor{black}{0.992} & \textcolor{black}{0.990} & \textcolor{black}{0.990} & \textcolor{black}{0.989} & \textcolor{black}{0.989} & \textcolor{black}{0.989} & \textcolor{black}{0.987} & \textcolor{black}{0.986}\\
oct$(struc)$ & \textcolor{black}{0.986} & \textcolor{black}{0.965} & \textcolor{black}{0.964} & \textcolor{black}{0.964} & \textcolor{black}{0.963} & \textcolor{black}{0.986} & \textcolor{black}{0.961} & \textcolor{black}{0.960} & \textcolor{black}{0.959} & \textcolor{black}{0.957}\\
oct$(wlsv)$ & \textcolor{black}{0.990} & \textcolor{black}{0.962} & \textcolor{black}{0.961} & \textcolor{black}{0.961} & \textcolor{black}{0.960} & \textcolor{red}{1.001} & \textcolor{black}{0.960} & \textcolor{black}{0.959} & \textcolor{black}{0.958} & \textcolor{black}{0.957}\\
oct$(bdshr)$ & \textcolor{black}{0.977} & \textcolor{black}{\textbf{0.959}} & \textcolor{black}{\textbf{0.956}} & \textcolor{black}{\textbf{0.955}} & \textcolor{blue}{\textbf{0.954}} & \textcolor{black}{0.985} & \textcolor{black}{\textbf{0.956}} & \textcolor{black}{\textbf{0.953}} & \textcolor{black}{\textbf{0.950}} & \textcolor{blue}{\textbf{0.948}}\\
oct$_h(hbshr)$ & \textcolor{black}{0.993} & \textcolor{red}{1.021} & \textcolor{red}{1.023} & \textcolor{red}{1.019} & \textcolor{red}{1.021} & \textcolor{black}{0.989} & \textcolor{red}{1.024} & \textcolor{red}{1.026} & \textcolor{red}{1.022} & \textcolor{red}{1.022}\\
oct$_h(bshr)$ & \textcolor{black}{0.997} & \textcolor{red}{1.022} & \textcolor{red}{1.022} & \textcolor{red}{1.019} & \textcolor{red}{1.022} & \textcolor{black}{0.994} & \textcolor{red}{1.022} & \textcolor{red}{1.022} & \textcolor{red}{1.020} & \textcolor{red}{1.022}\\
oct$_h(hshr)$ & \textcolor{black}{\textbf{0.973}} & \textcolor{black}{0.996} & \textcolor{black}{0.997} & \textcolor{black}{0.994} & \textcolor{black}{0.995} & \textcolor{black}{\textbf{0.976}} & \textcolor{black}{1.000} & \textcolor{red}{1.001} & \textcolor{black}{0.996} & \textcolor{black}{0.997}\\
oct$_h(shr)$ & \textcolor{red}{1.009} & \textcolor{black}{0.984} & \textcolor{black}{0.976} & \textcolor{black}{0.973} & \textcolor{black}{0.973} & \textcolor{red}{1.010} & \textcolor{black}{0.978} & \textcolor{black}{0.970} & \textcolor{black}{0.967} & \textcolor{black}{0.967}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 12$}} & \multicolumn{5}{c}{}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.968} & \textcolor{black}{0.967} & \textcolor{black}{0.969} & \textcolor{black}{0.969} &  &  &  &  & \\
ct$(bu)$ & \textcolor{red}{1.675} & \textcolor{red}{1.038} & \textcolor{red}{1.037} & \textcolor{red}{1.037} & \textcolor{red}{1.038} &  &  &  &  & \\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.163} & \textcolor{black}{0.977} & \textcolor{black}{0.965} & \textcolor{black}{0.977} & \textcolor{black}{0.965} &  &  &  &  & \\
ct$(wlsv_{te}, bu_{cs})$ & \textcolor{red}{1.174} & \textcolor{black}{0.978} & \textcolor{black}{0.978} & \textcolor{black}{0.971} & \textcolor{black}{0.971} &  &  &  &  & \\
oct$(ols)$ & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.983} & \textcolor{black}{0.980} & \textcolor{black}{0.975} &  &  &  &  & \\
oct$(struc)$ & \textcolor{black}{0.982} & \textcolor{black}{0.951} & \textcolor{black}{0.949} & \textcolor{black}{0.947} & \textcolor{black}{0.943} &  &  &  &  & \\
oct$(wlsv)$ & \textcolor{red}{1.025} & \textcolor{black}{0.954} & \textcolor{black}{0.953} & \textcolor{black}{0.949} & \textcolor{black}{0.947} &  &  &  &  & \\
oct$(bdshr)$ & \textcolor{red}{1.002} & \textcolor{black}{\textbf{0.950}} & \textcolor{black}{\textbf{0.944}} & \textcolor{black}{\textbf{0.939}} & \textcolor{blue}{\textbf{0.935}} &  &  &  &  & \\
oct$_h(hbshr)$ & \textcolor{black}{0.982} & \textcolor{red}{1.027} & \textcolor{red}{1.029} & \textcolor{red}{1.024} & \textcolor{red}{1.021} &  &  &  &  & \\
oct$_h(bshr)$ & \textcolor{black}{0.987} & \textcolor{red}{1.024} & \textcolor{red}{1.021} & \textcolor{red}{1.021} & \textcolor{red}{1.019} &  &  &  &  & \\
oct$_h(hshr)$ & \textcolor{black}{\textbf{0.978}} & \textcolor{red}{1.003} & \textcolor{red}{1.005} & \textcolor{black}{0.996} & \textcolor{black}{0.997} &  &  &  &  & \\
oct$_h(shr)$ & \textcolor{red}{1.010} & \textcolor{black}{0.963} & \textcolor{black}{0.956} & \textcolor{black}{0.952} & \textcolor{black}{0.952} &  &  &  &  & \\
\bottomrule
\multicolumn{11}{l}{\rule{0pt}{1em}\rule{0pt}{1.75em}\makecell[l]{$^\ast$The Gaussian method employs a sample covariance matrix and includes four techniques\\ (G, B, H, HB) with multi-step residuals.}}\\
\end{tabular}


==> tab/VN525/sam_crps_part.tex <==

\begin{tabular}[t]{l|>{}cccc>{}c|ccccc}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{10}{c}{\textbf{Generation of the base forecasts sample paths}} \\
\cmidrule(l{0pt}r{0pt}){2-11}
\multicolumn{1}{c}{\makecell[c]{\bfseries Reconciliation\\\bfseries approach}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} \\
\multicolumn{1}{c}{} &  & G & B & H & \multicolumn{1}{c}{HB} &  & G & B & H & HB\\
\midrule
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$\forall k \in \{12,6,4,3,2,1\}$}} & \multicolumn{5}{c}{\textbf{$k = 1$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.971} & \textcolor{black}{0.971} & \textcolor{black}{0.973} & \textcolor{black}{0.973} & \textcolor{black}{1.000} & \textcolor{black}{0.972} & \textcolor{black}{0.972} & \textcolor{black}{0.972} & \textcolor{black}{0.972}\\
ct$(bu)$ & \textcolor{red}{1.321} & \textcolor{red}{1.011} & \textcolor{red}{1.011} & \textcolor{red}{1.011} & \textcolor{red}{1.011} & \textcolor{red}{1.077} & \textcolor{black}{0.983} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.982}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.057} & \textcolor{black}{0.974} & \textcolor{black}{0.969} & \textcolor{black}{0.974} & \textcolor{black}{0.969} & \textcolor{black}{0.976} & \textcolor{black}{0.963} & \textcolor{black}{0.962} & \textcolor{black}{0.963} & \textcolor{black}{0.962}\\
ct$(wlsv_{te}, bu_{cs})$ & \textcolor{red}{1.062} & \textcolor{black}{0.974} & \textcolor{black}{0.974} & \textcolor{black}{0.972} & \textcolor{black}{0.972} & \textcolor{black}{0.976} & \textcolor{black}{0.965} & \textcolor{black}{0.965} & \textcolor{black}{0.966} & \textcolor{black}{0.966}\\
oct$(ols)$ & \textcolor{black}{0.989} & \textcolor{black}{0.989} & \textcolor{black}{0.989} & \textcolor{black}{0.987} & \textcolor{black}{0.987} & \textcolor{black}{0.982} & \textcolor{black}{0.986} & \textcolor{black}{0.988} & \textcolor{black}{0.986} & \textcolor{black}{0.989}\\
oct$(struc)$ & \textcolor{black}{0.982} & \textcolor{black}{0.962} & \textcolor{black}{0.961} & \textcolor{black}{0.961} & \textcolor{black}{0.959} & \textcolor{black}{0.970} & \textcolor{black}{0.963} & \textcolor{black}{0.963} & \textcolor{black}{0.963} & \textcolor{black}{0.963}\\
oct$(wlsv)$ & \textcolor{black}{0.987} & \textcolor{black}{0.959} & \textcolor{black}{0.959} & \textcolor{black}{0.958} & \textcolor{black}{0.957} & \textcolor{black}{0.952} & \textcolor{black}{0.957} & \textcolor{black}{0.957} & \textcolor{black}{0.957} & \textcolor{black}{0.957}\\
oct$(bdshr)$ & \textcolor{black}{0.975} & \textcolor{black}{\textbf{0.956}} & \textcolor{black}{\textbf{0.953}} & \textcolor{black}{\textbf{0.952}} & \textcolor{blue}{\textbf{0.951}} & \textcolor{blue}{\textbf{0.949}} & \textcolor{black}{\textbf{0.955}} & \textcolor{black}{\textbf{0.953}} & \textcolor{black}{\textbf{0.954}} & \textcolor{black}{\textbf{0.954}}\\
oct$_h(hbshr)$ & \textcolor{black}{0.989} & \textcolor{red}{1.018} & \textcolor{red}{1.020} & \textcolor{red}{1.016} & \textcolor{red}{1.018} & \textcolor{black}{0.982} & \textcolor{red}{1.004} & \textcolor{red}{1.007} & \textcolor{red}{1.004} & \textcolor{red}{1.009}\\
oct$_h(bshr)$ & \textcolor{black}{0.994} & \textcolor{red}{1.018} & \textcolor{red}{1.020} & \textcolor{red}{1.016} & \textcolor{red}{1.019} & \textcolor{black}{0.988} & \textcolor{red}{1.007} & \textcolor{red}{1.013} & \textcolor{red}{1.006} & \textcolor{red}{1.012}\\
oct$_h(hshr)$ & \textcolor{black}{\textbf{0.969}} & \textcolor{black}{0.993} & \textcolor{black}{0.993} & \textcolor{black}{0.990} & \textcolor{black}{0.991} & \textcolor{black}{0.953} & \textcolor{black}{0.977} & \textcolor{black}{0.977} & \textcolor{black}{0.979} & \textcolor{black}{0.979}\\
oct$_h(shr)$ & \textcolor{red}{1.007} & \textcolor{black}{0.980} & \textcolor{black}{0.972} & \textcolor{black}{0.970} & \textcolor{black}{0.970} & \textcolor{red}{1.000} & \textcolor{black}{0.986} & \textcolor{black}{0.977} & \textcolor{black}{0.976} & \textcolor{black}{0.974}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 3$}} & \multicolumn{5}{c}{\textbf{$k = 12$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.971} & \textcolor{black}{0.971} & \textcolor{black}{0.972} & \textcolor{black}{0.973} & \textcolor{black}{1.000} & \textcolor{black}{0.968} & \textcolor{black}{0.967} & \textcolor{black}{0.969} & \textcolor{black}{0.969}\\
ct$(bu)$ & \textcolor{red}{1.273} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.675} & \textcolor{red}{1.038} & \textcolor{red}{1.037} & \textcolor{red}{1.037} & \textcolor{red}{1.038}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.041} & \textcolor{black}{0.977} & \textcolor{black}{0.974} & \textcolor{black}{0.977} & \textcolor{black}{0.974} & \textcolor{red}{1.163} & \textcolor{black}{0.977} & \textcolor{black}{0.965} & \textcolor{black}{0.977} & \textcolor{black}{0.965}\\
ct$(wlsv_{te}, bu_{cs})$ & \textcolor{red}{1.046} & \textcolor{black}{0.976} & \textcolor{black}{0.976} & \textcolor{black}{0.974} & \textcolor{black}{0.974} & \textcolor{red}{1.174} & \textcolor{black}{0.978} & \textcolor{black}{0.978} & \textcolor{black}{0.971} & \textcolor{black}{0.971}\\
oct$(ols)$ & \textcolor{black}{0.994} & \textcolor{black}{0.992} & \textcolor{black}{0.993} & \textcolor{black}{0.991} & \textcolor{black}{0.992} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.983} & \textcolor{black}{0.980} & \textcolor{black}{0.975}\\
oct$(struc)$ & \textcolor{black}{0.986} & \textcolor{black}{0.967} & \textcolor{black}{0.966} & \textcolor{black}{0.966} & \textcolor{black}{0.965} & \textcolor{black}{0.982} & \textcolor{black}{0.951} & \textcolor{black}{0.949} & \textcolor{black}{0.947} & \textcolor{black}{0.943}\\
oct$(wlsv)$ & \textcolor{black}{0.983} & \textcolor{black}{0.963} & \textcolor{black}{0.962} & \textcolor{black}{0.962} & \textcolor{black}{0.962} & \textcolor{red}{1.025} & \textcolor{black}{0.954} & \textcolor{black}{0.953} & \textcolor{black}{0.949} & \textcolor{black}{0.947}\\
oct$(bdshr)$ & \textcolor{black}{0.972} & \textcolor{black}{\textbf{0.960}} & \textcolor{black}{\textbf{0.958}} & \textcolor{black}{\textbf{0.957}} & \textcolor{blue}{\textbf{0.957}} & \textcolor{red}{1.002} & \textcolor{black}{\textbf{0.950}} & \textcolor{black}{\textbf{0.944}} & \textcolor{black}{\textbf{0.939}} & \textcolor{blue}{\textbf{0.935}}\\
oct$_h(hbshr)$ & \textcolor{black}{0.994} & \textcolor{red}{1.019} & \textcolor{red}{1.021} & \textcolor{red}{1.018} & \textcolor{red}{1.020} & \textcolor{black}{0.982} & \textcolor{red}{1.027} & \textcolor{red}{1.029} & \textcolor{red}{1.024} & \textcolor{red}{1.021}\\
oct$_h(bshr)$ & \textcolor{black}{0.999} & \textcolor{red}{1.021} & \textcolor{red}{1.022} & \textcolor{red}{1.018} & \textcolor{red}{1.022} & \textcolor{black}{0.987} & \textcolor{red}{1.024} & \textcolor{red}{1.021} & \textcolor{red}{1.021} & \textcolor{red}{1.019}\\
oct$_h(hshr)$ & \textcolor{black}{\textbf{0.971}} & \textcolor{black}{0.994} & \textcolor{black}{0.994} & \textcolor{black}{0.992} & \textcolor{black}{0.993} & \textcolor{black}{\textbf{0.978}} & \textcolor{red}{1.003} & \textcolor{red}{1.005} & \textcolor{black}{0.996} & \textcolor{black}{0.997}\\
oct$_h(shr)$ & \textcolor{red}{1.009} & \textcolor{black}{0.986} & \textcolor{black}{0.978} & \textcolor{black}{0.976} & \textcolor{black}{0.976} & \textcolor{red}{1.010} & \textcolor{black}{0.963} & \textcolor{black}{0.956} & \textcolor{black}{0.952} & \textcolor{black}{0.952}\\
\bottomrule
\multicolumn{11}{l}{\rule{0pt}{1em}\rule{0pt}{1.75em}\makecell[l]{$^\ast$The Gaussian method employs a sample covariance matrix and includes four techniques\\ (G, B, H, HB) with multi-step residuals.}}\\
\end{tabular}


==> tab/VN525/sam_es_more.tex <==

\begin{tabular}[t]{c|>{}cccc>{}c|ccccc}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{10}{c}{\textbf{Base forecasts' sample approach}} \\
\cmidrule(l{0pt}r{0pt}){2-11}
\multicolumn{1}{c}{\makecell[c]{\bfseries Reconciliation\\\bfseries approach}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} \\
\multicolumn{1}{c}{} &  & G & B & H & \multicolumn{1}{c}{HB} &  & G & B & H & HB\\
\midrule
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$\forall k \in \{12,6,4,3,2,1\}$}} & \multicolumn{5}{c}{\textbf{$k = 1$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.956} & \textcolor{black}{0.955} & \textcolor{black}{0.958} & \textcolor{black}{0.951} & \textcolor{black}{1.000} & \textcolor{black}{0.952} & \textcolor{black}{0.950} & \textcolor{black}{0.952} & \textcolor{black}{0.950}\\
ct$(bu)$ & \textcolor{red}{2.427} & \textcolor{black}{0.983} & \textcolor{black}{0.983} & \textcolor{black}{0.983} & \textcolor{black}{0.983} & \textcolor{red}{1.759} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.982}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.243} & \textcolor{black}{0.886} & \textcolor{black}{0.879} & \textcolor{black}{0.886} & \textcolor{black}{0.879} & \textcolor{red}{1.098} & \textcolor{black}{0.929} & \textcolor{black}{0.928} & \textcolor{black}{0.930} & \textcolor{black}{0.927}\\
ct$(wlsv_{te}, bu_{cs})$ & \textcolor{red}{1.499} & \textcolor{black}{0.977} & \textcolor{black}{0.977} & \textcolor{black}{0.971} & \textcolor{black}{0.972} & \textcolor{red}{1.241} & \textcolor{black}{0.975} & \textcolor{black}{0.975} & \textcolor{black}{0.973} & \textcolor{black}{0.974}\\
oct$(ols)$ & \textcolor{black}{0.955} & \textcolor{black}{0.893} & \textcolor{black}{0.891} & \textcolor{black}{0.893} & \textcolor{black}{0.888} & \textcolor{black}{0.975} & \textcolor{black}{0.937} & \textcolor{black}{0.936} & \textcolor{black}{0.936} & \textcolor{black}{0.935}\\
oct$(struc)$ & \textcolor{red}{1.085} & \textcolor{black}{0.917} & \textcolor{black}{0.915} & \textcolor{black}{0.916} & \textcolor{black}{0.912} & \textcolor{red}{1.027} & \textcolor{black}{0.943} & \textcolor{black}{0.942} & \textcolor{black}{0.943} & \textcolor{black}{0.942}\\
oct$(wlsv)$ & \textcolor{red}{1.132} & \textcolor{black}{0.933} & \textcolor{black}{0.929} & \textcolor{black}{0.931} & \textcolor{black}{0.927} & \textcolor{red}{1.050} & \textcolor{black}{0.951} & \textcolor{black}{0.949} & \textcolor{black}{0.950} & \textcolor{black}{0.949}\\
oct$(bdshr)$ & \textcolor{red}{1.047} & \textcolor{black}{0.904} & \textcolor{black}{0.897} & \textcolor{black}{0.897} & \textcolor{black}{0.891} & \textcolor{red}{1.009} & \textcolor{black}{0.936} & \textcolor{black}{0.933} & \textcolor{black}{0.934} & \textcolor{black}{0.931}\\
oct$_h(hbshr)$ & \textcolor{black}{0.956} & \textcolor{black}{0.889} & \textcolor{black}{0.886} & \textcolor{black}{0.888} & \textcolor{black}{0.884} & \textcolor{black}{0.975} & \textcolor{black}{0.937} & \textcolor{black}{0.936} & \textcolor{black}{0.937} & \textcolor{black}{0.935}\\
oct$_h(bshr)$ & \textcolor{black}{\textbf{0.931}} & \textcolor{black}{\textbf{0.867}} & \textcolor{black}{\textbf{0.866}} & \textcolor{black}{\textbf{0.863}} & \textcolor{blue}{\textbf{0.860}} & \textcolor{black}{\textbf{0.965}} & \textcolor{black}{\textbf{0.927}} & \textcolor{black}{0.927} & \textcolor{black}{0.925} & \textcolor{black}{0.923}\\
oct$_h(hshr)$ & \textcolor{red}{1.081} & \textcolor{black}{0.935} & \textcolor{black}{0.931} & \textcolor{black}{0.935} & \textcolor{black}{0.927} & \textcolor{red}{1.028} & \textcolor{black}{0.952} & \textcolor{black}{0.951} & \textcolor{black}{0.952} & \textcolor{black}{0.950}\\
oct$_h(shr)$ & \textcolor{red}{1.068} & \textcolor{black}{0.899} & \textcolor{black}{0.878} & \textcolor{black}{0.875} & \textcolor{black}{0.864} & \textcolor{red}{1.023} & \textcolor{black}{0.935} & \textcolor{black}{\textbf{0.923}} & \textcolor{black}{\textbf{0.921}} & \textcolor{blue}{\textbf{0.916}}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 2$}} & \multicolumn{5}{c}{\textbf{$k = 3$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.958} & \textcolor{black}{0.954} & \textcolor{black}{0.956} & \textcolor{black}{0.953} & \textcolor{black}{1.000} & \textcolor{black}{0.961} & \textcolor{black}{0.958} & \textcolor{black}{0.960} & \textcolor{black}{0.955}\\
ct$(bu)$ & \textcolor{red}{2.176} & \textcolor{red}{1.001} & \textcolor{red}{1.001} & \textcolor{red}{1.001} & \textcolor{red}{1.001} & \textcolor{red}{2.428} & \textcolor{black}{0.998} & \textcolor{black}{0.997} & \textcolor{black}{0.997} & \textcolor{black}{0.997}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.192} & \textcolor{black}{0.927} & \textcolor{black}{0.921} & \textcolor{black}{0.927} & \textcolor{black}{0.921} & \textcolor{red}{1.245} & \textcolor{black}{0.911} & \textcolor{black}{0.904} & \textcolor{black}{0.911} & \textcolor{black}{0.904}\\
ct$(wlsv_{te}, bu_{cs})$ & \textcolor{red}{1.400} & \textcolor{black}{0.992} & \textcolor{black}{0.992} & \textcolor{black}{0.988} & \textcolor{black}{0.988} & \textcolor{red}{1.500} & \textcolor{black}{0.991} & \textcolor{black}{0.991} & \textcolor{black}{0.986} & \textcolor{black}{0.987}\\
oct$(ols)$ & \textcolor{black}{0.985} & \textcolor{black}{0.935} & \textcolor{black}{0.932} & \textcolor{black}{0.934} & \textcolor{black}{0.930} & \textcolor{black}{0.976} & \textcolor{black}{0.918} & \textcolor{black}{0.915} & \textcolor{black}{0.917} & \textcolor{black}{0.912}\\
oct$(struc)$ & \textcolor{red}{1.075} & \textcolor{black}{0.949} & \textcolor{black}{0.947} & \textcolor{black}{0.948} & \textcolor{black}{0.944} & \textcolor{red}{1.096} & \textcolor{black}{0.939} & \textcolor{black}{0.936} & \textcolor{black}{0.938} & \textcolor{black}{0.933}\\
oct$(wlsv)$ & \textcolor{red}{1.110} & \textcolor{black}{0.960} & \textcolor{black}{0.958} & \textcolor{black}{0.958} & \textcolor{black}{0.955} & \textcolor{red}{1.142} & \textcolor{black}{0.953} & \textcolor{black}{0.949} & \textcolor{black}{0.951} & \textcolor{black}{0.946}\\
oct$(bdshr)$ & \textcolor{red}{1.045} & \textcolor{black}{0.938} & \textcolor{black}{0.933} & \textcolor{black}{0.933} & \textcolor{black}{0.929} & \textcolor{red}{1.060} & \textcolor{black}{0.926} & \textcolor{black}{0.920} & \textcolor{black}{0.921} & \textcolor{black}{0.915}\\
oct$_h(hbshr)$ & \textcolor{black}{0.984} & \textcolor{black}{0.933} & \textcolor{black}{0.931} & \textcolor{black}{0.933} & \textcolor{black}{0.928} & \textcolor{black}{0.975} & \textcolor{black}{0.915} & \textcolor{black}{0.912} & \textcolor{black}{0.915} & \textcolor{black}{0.909}\\
oct$_h(bshr)$ & \textcolor{black}{\textbf{0.967}} & \textcolor{black}{\textbf{0.917}} & \textcolor{black}{\textbf{0.916}} & \textcolor{black}{0.913} & \textcolor{black}{0.908} & \textcolor{black}{\textbf{0.954}} & \textcolor{black}{\textbf{0.895}} & \textcolor{black}{\textbf{0.895}} & \textcolor{black}{\textbf{0.892}} & \textcolor{blue}{\textbf{0.887}}\\
oct$_h(hshr)$ & \textcolor{red}{1.073} & \textcolor{black}{0.962} & \textcolor{black}{0.959} & \textcolor{black}{0.963} & \textcolor{black}{0.956} & \textcolor{red}{1.093} & \textcolor{black}{0.955} & \textcolor{black}{0.951} & \textcolor{black}{0.956} & \textcolor{black}{0.949}\\
oct$_h(shr)$ & \textcolor{red}{1.064} & \textcolor{black}{0.933} & \textcolor{black}{0.916} & \textcolor{black}{\textbf{0.913}} & \textcolor{blue}{\textbf{0.904}} & \textcolor{red}{1.082} & \textcolor{black}{0.923} & \textcolor{black}{0.903} & \textcolor{black}{0.900} & \textcolor{black}{0.890}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 4$}} & \multicolumn{5}{c}{\textbf{$k = 6$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.960} & \textcolor{black}{0.960} & \textcolor{black}{0.962} & \textcolor{black}{0.956} & \textcolor{black}{1.000} & \textcolor{black}{0.961} & \textcolor{black}{0.959} & \textcolor{black}{0.964} & \textcolor{black}{0.956}\\
ct$(bu)$ & \textcolor{red}{2.585} & \textcolor{black}{0.996} & \textcolor{black}{0.996} & \textcolor{black}{0.995} & \textcolor{black}{0.996} & \textcolor{red}{2.849} & \textcolor{red}{1.004} & \textcolor{red}{1.003} & \textcolor{red}{1.003} & \textcolor{red}{1.004}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.277} & \textcolor{black}{0.898} & \textcolor{black}{0.890} & \textcolor{black}{0.899} & \textcolor{black}{0.891} & \textcolor{red}{1.339} & \textcolor{black}{0.882} & \textcolor{black}{0.873} & \textcolor{black}{0.883} & \textcolor{black}{0.874}\\
ct$(wlsv_{te}, bu_{cs})$ & \textcolor{red}{1.559} & \textcolor{black}{0.990} & \textcolor{black}{0.990} & \textcolor{black}{0.984} & \textcolor{black}{0.985} & \textcolor{red}{1.662} & \textcolor{black}{0.997} & \textcolor{black}{0.997} & \textcolor{black}{0.991} & \textcolor{black}{0.992}\\
oct$(ols)$ & \textcolor{black}{0.966} & \textcolor{black}{0.905} & \textcolor{black}{0.902} & \textcolor{black}{0.904} & \textcolor{black}{0.899} & \textcolor{black}{0.962} & \textcolor{black}{0.889} & \textcolor{black}{0.887} & \textcolor{black}{0.890} & \textcolor{black}{0.885}\\
oct$(struc)$ & \textcolor{red}{1.106} & \textcolor{black}{0.930} & \textcolor{black}{0.927} & \textcolor{black}{0.928} & \textcolor{black}{0.924} & \textcolor{red}{1.132} & \textcolor{black}{0.923} & \textcolor{black}{0.919} & \textcolor{black}{0.922} & \textcolor{black}{0.916}\\
oct$(wlsv)$ & \textcolor{red}{1.157} & \textcolor{black}{0.947} & \textcolor{black}{0.943} & \textcolor{black}{0.945} & \textcolor{black}{0.939} & \textcolor{red}{1.192} & \textcolor{black}{0.942} & \textcolor{black}{0.937} & \textcolor{black}{0.941} & \textcolor{black}{0.934}\\
oct$(bdshr)$ & \textcolor{red}{1.065} & \textcolor{black}{0.917} & \textcolor{black}{0.909} & \textcolor{black}{0.910} & \textcolor{black}{0.903} & \textcolor{red}{1.084} & \textcolor{black}{0.907} & \textcolor{black}{0.897} & \textcolor{black}{0.898} & \textcolor{black}{0.890}\\
oct$_h(hbshr)$ & \textcolor{black}{0.967} & \textcolor{black}{0.901} & \textcolor{black}{0.898} & \textcolor{black}{0.900} & \textcolor{black}{0.895} & \textcolor{black}{0.964} & \textcolor{black}{0.882} & \textcolor{black}{0.880} & \textcolor{black}{0.883} & \textcolor{black}{0.877}\\
oct$_h(bshr)$ & \textcolor{black}{\textbf{0.943}} & \textcolor{black}{\textbf{0.879}} & \textcolor{black}{\textbf{0.878}} & \textcolor{black}{\textbf{0.876}} & \textcolor{blue}{\textbf{0.871}} & \textcolor{black}{\textbf{0.932}} & \textcolor{black}{\textbf{0.856}} & \textcolor{black}{\textbf{0.855}} & \textcolor{black}{\textbf{0.851}} & \textcolor{blue}{\textbf{0.848}}\\
oct$_h(hshr)$ & \textcolor{red}{1.101} & \textcolor{black}{0.949} & \textcolor{black}{0.944} & \textcolor{black}{0.949} & \textcolor{black}{0.941} & \textcolor{red}{1.126} & \textcolor{black}{0.945} & \textcolor{black}{0.939} & \textcolor{black}{0.945} & \textcolor{black}{0.936}\\
oct$_h(shr)$ & \textcolor{red}{1.089} & \textcolor{black}{0.915} & \textcolor{black}{0.893} & \textcolor{black}{0.890} & \textcolor{black}{0.878} & \textcolor{red}{1.107} & \textcolor{black}{0.899} & \textcolor{black}{0.875} & \textcolor{black}{0.871} & \textcolor{black}{0.858}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 12$}} & \multicolumn{5}{c}{}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.942} & \textcolor{black}{0.947} & \textcolor{black}{0.951} & \textcolor{black}{0.937} &  &  &  &  & \\
ct$(bu)$ & \textcolor{red}{2.990} & \textcolor{black}{0.922} & \textcolor{black}{0.921} & \textcolor{black}{0.923} & \textcolor{black}{0.923} &  &  &  &  & \\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.326} & \textcolor{black}{0.779} & \textcolor{black}{0.767} & \textcolor{black}{0.777} & \textcolor{black}{0.766} &  &  &  &  & \\
ct$(wlsv_{te}, bu_{cs})$ & \textcolor{red}{1.679} & \textcolor{black}{0.917} & \textcolor{black}{0.917} & \textcolor{black}{0.906} & \textcolor{black}{0.908} &  &  &  &  & \\
oct$(ols)$ & \textcolor{black}{0.872} & \textcolor{black}{0.783} & \textcolor{black}{0.784} & \textcolor{black}{0.783} & \textcolor{black}{0.779} &  &  &  &  & \\
oct$(struc)$ & \textcolor{red}{1.077} & \textcolor{black}{0.826} & \textcolor{black}{0.822} & \textcolor{black}{0.823} & \textcolor{black}{0.818} &  &  &  &  & \\
oct$(wlsv)$ & \textcolor{red}{1.149} & \textcolor{black}{0.851} & \textcolor{black}{0.845} & \textcolor{black}{0.847} & \textcolor{black}{0.840} &  &  &  &  & \\
oct$(bdshr)$ & \textcolor{red}{1.021} & \textcolor{black}{0.808} & \textcolor{black}{0.796} & \textcolor{black}{0.796} & \textcolor{black}{0.787} &  &  &  &  & \\
oct$_h(hbshr)$ & \textcolor{black}{0.872} & \textcolor{black}{0.775} & \textcolor{black}{0.772} & \textcolor{black}{0.772} & \textcolor{black}{0.770} &  &  &  &  & \\
oct$_h(bshr)$ & \textcolor{black}{\textbf{0.833}} & \textcolor{black}{\textbf{0.741}} & \textcolor{black}{\textbf{0.741}} & \textcolor{black}{\textbf{0.737}} & \textcolor{blue}{\textbf{0.735}} &  &  &  &  & \\
oct$_h(hshr)$ & \textcolor{red}{1.066} & \textcolor{black}{0.851} & \textcolor{black}{0.846} & \textcolor{black}{0.848} & \textcolor{black}{0.838} &  &  &  &  & \\
oct$_h(shr)$ & \textcolor{red}{1.043} & \textcolor{black}{0.797} & \textcolor{black}{0.768} & \textcolor{black}{0.764} & \textcolor{black}{0.750} &  &  &  &  & \\
\bottomrule
\multicolumn{11}{l}{\rule{0pt}{1em}\rule{0pt}{1.75em}\makecell[l]{$^\ast$The Gaussian method employs a sample covariance matrix and includes four techniques\\ (G, B, H, HB) with multi-step residuals.}}\\
\end{tabular}


==> tab/VN525/sam_es_part.tex <==

\begin{tabular}[t]{l|>{}cccc>{}c|ccccc}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{10}{c}{\textbf{Generation of the base forecasts sample paths}} \\
\cmidrule(l{0pt}r{0pt}){2-11}
\multicolumn{1}{c}{\makecell[c]{\bfseries Reconciliation\\\bfseries approach}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} \\
\multicolumn{1}{c}{} &  & G & B & H & \multicolumn{1}{c}{HB} &  & G & B & H & HB\\
\midrule
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$\forall k \in \{12,6,4,3,2,1\}$}} & \multicolumn{5}{c}{\textbf{$k = 1$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.956} & \textcolor{black}{0.955} & \textcolor{black}{0.958} & \textcolor{black}{0.951} & \textcolor{black}{1.000} & \textcolor{black}{0.952} & \textcolor{black}{0.950} & \textcolor{black}{0.952} & \textcolor{black}{0.950}\\
ct$(bu)$ & \textcolor{red}{2.427} & \textcolor{black}{0.983} & \textcolor{black}{0.983} & \textcolor{black}{0.983} & \textcolor{black}{0.983} & \textcolor{red}{1.759} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.982}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.243} & \textcolor{black}{0.886} & \textcolor{black}{0.879} & \textcolor{black}{0.886} & \textcolor{black}{0.879} & \textcolor{red}{1.098} & \textcolor{black}{0.929} & \textcolor{black}{0.928} & \textcolor{black}{0.930} & \textcolor{black}{0.927}\\
ct$(wlsv_{te}, bu_{cs})$ & \textcolor{red}{1.499} & \textcolor{black}{0.977} & \textcolor{black}{0.977} & \textcolor{black}{0.971} & \textcolor{black}{0.972} & \textcolor{red}{1.241} & \textcolor{black}{0.975} & \textcolor{black}{0.975} & \textcolor{black}{0.973} & \textcolor{black}{0.974}\\
oct$(ols)$ & \textcolor{black}{0.955} & \textcolor{black}{0.893} & \textcolor{black}{0.891} & \textcolor{black}{0.893} & \textcolor{black}{0.888} & \textcolor{black}{0.975} & \textcolor{black}{0.937} & \textcolor{black}{0.936} & \textcolor{black}{0.936} & \textcolor{black}{0.935}\\
oct$(struc)$ & \textcolor{red}{1.085} & \textcolor{black}{0.917} & \textcolor{black}{0.915} & \textcolor{black}{0.916} & \textcolor{black}{0.912} & \textcolor{red}{1.027} & \textcolor{black}{0.943} & \textcolor{black}{0.942} & \textcolor{black}{0.943} & \textcolor{black}{0.942}\\
oct$(wlsv)$ & \textcolor{red}{1.132} & \textcolor{black}{0.933} & \textcolor{black}{0.929} & \textcolor{black}{0.931} & \textcolor{black}{0.927} & \textcolor{red}{1.050} & \textcolor{black}{0.951} & \textcolor{black}{0.949} & \textcolor{black}{0.950} & \textcolor{black}{0.949}\\
oct$(bdshr)$ & \textcolor{red}{1.047} & \textcolor{black}{0.904} & \textcolor{black}{0.897} & \textcolor{black}{0.897} & \textcolor{black}{0.891} & \textcolor{red}{1.009} & \textcolor{black}{0.936} & \textcolor{black}{0.933} & \textcolor{black}{0.934} & \textcolor{black}{0.931}\\
oct$_h(hbshr)$ & \textcolor{black}{0.956} & \textcolor{black}{0.889} & \textcolor{black}{0.886} & \textcolor{black}{0.888} & \textcolor{black}{0.884} & \textcolor{black}{0.975} & \textcolor{black}{0.937} & \textcolor{black}{0.936} & \textcolor{black}{0.937} & \textcolor{black}{0.935}\\
oct$_h(bshr)$ & \textcolor{black}{\textbf{0.931}} & \textcolor{black}{\textbf{0.867}} & \textcolor{black}{\textbf{0.866}} & \textcolor{black}{\textbf{0.863}} & \textcolor{blue}{\textbf{0.860}} & \textcolor{black}{\textbf{0.965}} & \textcolor{black}{\textbf{0.927}} & \textcolor{black}{0.927} & \textcolor{black}{0.925} & \textcolor{black}{0.923}\\
oct$_h(hshr)$ & \textcolor{red}{1.081} & \textcolor{black}{0.935} & \textcolor{black}{0.931} & \textcolor{black}{0.935} & \textcolor{black}{0.927} & \textcolor{red}{1.028} & \textcolor{black}{0.952} & \textcolor{black}{0.951} & \textcolor{black}{0.952} & \textcolor{black}{0.950}\\
oct$_h(shr)$ & \textcolor{red}{1.068} & \textcolor{black}{0.899} & \textcolor{black}{0.878} & \textcolor{black}{0.875} & \textcolor{black}{0.864} & \textcolor{red}{1.023} & \textcolor{black}{0.935} & \textcolor{black}{\textbf{0.923}} & \textcolor{black}{\textbf{0.921}} & \textcolor{blue}{\textbf{0.916}}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 3$}} & \multicolumn{5}{c}{\textbf{$k = 12$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.961} & \textcolor{black}{0.958} & \textcolor{black}{0.960} & \textcolor{black}{0.955} & \textcolor{black}{1.000} & \textcolor{black}{0.942} & \textcolor{black}{0.947} & \textcolor{black}{0.951} & \textcolor{black}{0.937}\\
ct$(bu)$ & \textcolor{red}{2.428} & \textcolor{black}{0.998} & \textcolor{black}{0.997} & \textcolor{black}{0.997} & \textcolor{black}{0.997} & \textcolor{red}{2.990} & \textcolor{black}{0.922} & \textcolor{black}{0.921} & \textcolor{black}{0.923} & \textcolor{black}{0.923}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.245} & \textcolor{black}{0.911} & \textcolor{black}{0.904} & \textcolor{black}{0.911} & \textcolor{black}{0.904} & \textcolor{red}{1.326} & \textcolor{black}{0.779} & \textcolor{black}{0.767} & \textcolor{black}{0.777} & \textcolor{black}{0.766}\\
ct$(wlsv_{te}, bu_{cs})$ & \textcolor{red}{1.500} & \textcolor{black}{0.991} & \textcolor{black}{0.991} & \textcolor{black}{0.986} & \textcolor{black}{0.987} & \textcolor{red}{1.679} & \textcolor{black}{0.917} & \textcolor{black}{0.917} & \textcolor{black}{0.906} & \textcolor{black}{0.908}\\
oct$(ols)$ & \textcolor{black}{0.976} & \textcolor{black}{0.918} & \textcolor{black}{0.915} & \textcolor{black}{0.917} & \textcolor{black}{0.912} & \textcolor{black}{0.872} & \textcolor{black}{0.783} & \textcolor{black}{0.784} & \textcolor{black}{0.783} & \textcolor{black}{0.779}\\
oct$(struc)$ & \textcolor{red}{1.096} & \textcolor{black}{0.939} & \textcolor{black}{0.936} & \textcolor{black}{0.938} & \textcolor{black}{0.933} & \textcolor{red}{1.077} & \textcolor{black}{0.826} & \textcolor{black}{0.822} & \textcolor{black}{0.823} & \textcolor{black}{0.818}\\
oct$(wlsv)$ & \textcolor{red}{1.142} & \textcolor{black}{0.953} & \textcolor{black}{0.949} & \textcolor{black}{0.951} & \textcolor{black}{0.946} & \textcolor{red}{1.149} & \textcolor{black}{0.851} & \textcolor{black}{0.845} & \textcolor{black}{0.847} & \textcolor{black}{0.840}\\
oct$(bdshr)$ & \textcolor{red}{1.060} & \textcolor{black}{0.926} & \textcolor{black}{0.920} & \textcolor{black}{0.921} & \textcolor{black}{0.915} & \textcolor{red}{1.021} & \textcolor{black}{0.808} & \textcolor{black}{0.796} & \textcolor{black}{0.796} & \textcolor{black}{0.787}\\
oct$_h(hbshr)$ & \textcolor{black}{0.975} & \textcolor{black}{0.915} & \textcolor{black}{0.912} & \textcolor{black}{0.915} & \textcolor{black}{0.909} & \textcolor{black}{0.872} & \textcolor{black}{0.775} & \textcolor{black}{0.772} & \textcolor{black}{0.772} & \textcolor{black}{0.770}\\
oct$_h(bshr)$ & \textcolor{black}{\textbf{0.954}} & \textcolor{black}{\textbf{0.895}} & \textcolor{black}{\textbf{0.895}} & \textcolor{black}{\textbf{0.892}} & \textcolor{blue}{\textbf{0.887}} & \textcolor{black}{\textbf{0.833}} & \textcolor{black}{\textbf{0.741}} & \textcolor{black}{\textbf{0.741}} & \textcolor{black}{\textbf{0.737}} & \textcolor{blue}{\textbf{0.735}}\\
oct$_h(hshr)$ & \textcolor{red}{1.093} & \textcolor{black}{0.955} & \textcolor{black}{0.951} & \textcolor{black}{0.956} & \textcolor{black}{0.949} & \textcolor{red}{1.066} & \textcolor{black}{0.851} & \textcolor{black}{0.846} & \textcolor{black}{0.848} & \textcolor{black}{0.838}\\
oct$_h(shr)$ & \textcolor{red}{1.082} & \textcolor{black}{0.923} & \textcolor{black}{0.903} & \textcolor{black}{0.900} & \textcolor{black}{0.890} & \textcolor{red}{1.043} & \textcolor{black}{0.797} & \textcolor{black}{0.768} & \textcolor{black}{0.764} & \textcolor{black}{0.750}\\
\bottomrule
\multicolumn{11}{l}{\rule{0pt}{1em}\rule{0pt}{1.75em}\makecell[l]{$^\ast$The Gaussian method employs a sample covariance matrix and includes four techniques\\ (G, B, H, HB) with multi-step residuals.}}\\
\end{tabular}


==> tab/VN525/trash/sam_crps.tex <==

\begin{tabular}[t]{c|>{}cccc>{}c|ccccc}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{10}{c}{\textbf{Base forecasts' sample approach}} \\
\cmidrule(l{0pt}r{0pt}){2-11}
\multicolumn{1}{c}{\makecell[c]{\bfseries Reconciliation\\\bfseries approach}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} \\
\multicolumn{1}{c}{} &  & G & B & H & \multicolumn{1}{c}{HB} &  & G & B & H & HB\\
\midrule
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$\forall k \in \{12,6,4,3,2,1\}$}} & \multicolumn{5}{c}{\textbf{$k = 1$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.971} & \textcolor{black}{0.971} & \textcolor{black}{0.973} & \textcolor{black}{0.973} & \textcolor{black}{1.000} & \textcolor{black}{0.972} & \textcolor{black}{0.972} & \textcolor{black}{0.972} & \textcolor{black}{0.972}\\
ct$(bu)$ & \textcolor{red}{1.321} & \textcolor{red}{1.011} & \textcolor{red}{1.011} & \textcolor{red}{1.011} & \textcolor{red}{1.011} & \textcolor{red}{1.077} & \textcolor{black}{0.983} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.982}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.057} & \textcolor{black}{0.974} & \textcolor{black}{0.969} & \textcolor{black}{0.974} & \textcolor{black}{0.969} & \textcolor{black}{0.976} & \textcolor{black}{0.963} & \textcolor{black}{0.962} & \textcolor{black}{0.963} & \textcolor{black}{0.962}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.082} & \textcolor{black}{0.977} & \textcolor{black}{0.976} & \textcolor{black}{0.977} & \textcolor{black}{0.976} & \textcolor{black}{0.986} & \textcolor{black}{0.965} & \textcolor{black}{0.965} & \textcolor{black}{0.965} & \textcolor{black}{0.965}\\
oct$(wlsv)$ & \textcolor{black}{0.987} & \textcolor{black}{0.959} & \textcolor{black}{0.959} & \textcolor{black}{0.958} & \textcolor{black}{0.957} & \textcolor{black}{0.952} & \textcolor{black}{0.957} & \textcolor{black}{0.957} & \textcolor{black}{0.957} & \textcolor{black}{0.957}\\
oct$(bdshr)$ & \textcolor{black}{\textbf{0.975}} & \textcolor{black}{\textbf{0.956}} & \textcolor{black}{\textbf{0.953}} & \textcolor{black}{\textbf{0.952}} & \textcolor{blue}{\textbf{0.951}} & \textcolor{blue}{\textbf{0.949}} & \textcolor{black}{\textbf{0.955}} & \textcolor{black}{\textbf{0.953}} & \textcolor{black}{\textbf{0.954}} & \textcolor{black}{\textbf{0.954}}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 2$}} & \multicolumn{5}{c}{\textbf{$k = 3$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.970} & \textcolor{black}{0.969} & \textcolor{black}{0.970} & \textcolor{black}{0.971} & \textcolor{black}{1.000} & \textcolor{black}{0.971} & \textcolor{black}{0.971} & \textcolor{black}{0.972} & \textcolor{black}{0.973}\\
ct$(bu)$ & \textcolor{red}{1.189} & \textcolor{black}{0.999} & \textcolor{black}{0.999} & \textcolor{black}{0.999} & \textcolor{black}{0.999} & \textcolor{red}{1.273} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.010}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.015} & \textcolor{black}{0.972} & \textcolor{black}{0.970} & \textcolor{black}{0.972} & \textcolor{black}{0.970} & \textcolor{red}{1.041} & \textcolor{black}{0.977} & \textcolor{black}{0.974} & \textcolor{black}{0.977} & \textcolor{black}{0.974}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.031} & \textcolor{black}{0.975} & \textcolor{black}{0.974} & \textcolor{black}{0.975} & \textcolor{black}{0.974} & \textcolor{red}{1.062} & \textcolor{black}{0.980} & \textcolor{black}{0.979} & \textcolor{black}{0.980} & \textcolor{black}{0.979}\\
oct$(wlsv)$ & \textcolor{black}{0.972} & \textcolor{black}{0.961} & \textcolor{black}{0.960} & \textcolor{black}{0.960} & \textcolor{black}{0.960} & \textcolor{black}{0.983} & \textcolor{black}{0.963} & \textcolor{black}{0.962} & \textcolor{black}{0.962} & \textcolor{black}{0.962}\\
oct$(bdshr)$ & \textcolor{black}{\textbf{0.964}} & \textcolor{black}{\textbf{0.958}} & \textcolor{black}{\textbf{0.957}} & \textcolor{black}{\textbf{0.956}} & \textcolor{blue}{\textbf{0.956}} & \textcolor{black}{\textbf{0.972}} & \textcolor{black}{\textbf{0.960}} & \textcolor{black}{\textbf{0.958}} & \textcolor{black}{\textbf{0.957}} & \textcolor{blue}{\textbf{0.957}}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 4$}} & \multicolumn{5}{c}{\textbf{$k = 6$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.973} & \textcolor{black}{0.973} & \textcolor{black}{0.974} & \textcolor{black}{0.975} & \textcolor{black}{1.000} & \textcolor{black}{0.976} & \textcolor{black}{0.976} & \textcolor{black}{0.978} & \textcolor{black}{0.978}\\
ct$(bu)$ & \textcolor{red}{1.340} & \textcolor{red}{1.016} & \textcolor{red}{1.015} & \textcolor{red}{1.015} & \textcolor{red}{1.015} & \textcolor{red}{1.450} & \textcolor{red}{1.023} & \textcolor{red}{1.023} & \textcolor{red}{1.023} & \textcolor{red}{1.023}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.061} & \textcolor{black}{0.978} & \textcolor{black}{0.973} & \textcolor{black}{0.978} & \textcolor{black}{0.973} & \textcolor{red}{1.094} & \textcolor{black}{0.978} & \textcolor{black}{0.972} & \textcolor{black}{0.978} & \textcolor{black}{0.972}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.087} & \textcolor{black}{0.982} & \textcolor{black}{0.980} & \textcolor{black}{0.982} & \textcolor{black}{0.980} & \textcolor{red}{1.127} & \textcolor{black}{0.982} & \textcolor{black}{0.981} & \textcolor{black}{0.982} & \textcolor{black}{0.981}\\
oct$(wlsv)$ & \textcolor{black}{0.990} & \textcolor{black}{0.962} & \textcolor{black}{0.961} & \textcolor{black}{0.961} & \textcolor{black}{0.960} & \textcolor{red}{1.001} & \textcolor{black}{0.960} & \textcolor{black}{0.959} & \textcolor{black}{0.958} & \textcolor{black}{0.957}\\
oct$(bdshr)$ & \textcolor{black}{\textbf{0.977}} & \textcolor{black}{\textbf{0.959}} & \textcolor{black}{\textbf{0.956}} & \textcolor{black}{\textbf{0.955}} & \textcolor{blue}{\textbf{0.954}} & \textcolor{black}{\textbf{0.985}} & \textcolor{black}{\textbf{0.956}} & \textcolor{black}{\textbf{0.953}} & \textcolor{black}{\textbf{0.950}} & \textcolor{blue}{\textbf{0.948}}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 12$}} & \multicolumn{5}{c}{}\\
base & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{0.968} & \textcolor{black}{0.967} & \textcolor{black}{0.969} & \textcolor{black}{0.969} &  &  &  &  & \\
ct$(bu)$ & \textcolor{red}{1.675} & \textcolor{red}{1.038} & \textcolor{red}{1.037} & \textcolor{red}{1.037} & \textcolor{red}{1.038} &  &  &  &  & \\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.163} & \textcolor{black}{0.977} & \textcolor{black}{0.965} & \textcolor{black}{0.977} & \textcolor{black}{0.965} &  &  &  &  & \\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.212} & \textcolor{black}{0.980} & \textcolor{black}{0.976} & \textcolor{black}{0.980} & \textcolor{black}{0.976} &  &  &  &  & \\
oct$(wlsv)$ & \textcolor{red}{1.025} & \textcolor{black}{0.954} & \textcolor{black}{0.953} & \textcolor{black}{0.949} & \textcolor{black}{0.947} &  &  &  &  & \\
oct$(bdshr)$ & \textcolor{red}{1.002} & \textcolor{black}{\textbf{0.950}} & \textcolor{black}{\textbf{0.944}} & \textcolor{black}{\textbf{0.939}} & \textcolor{blue}{\textbf{0.935}} &  &  &  &  & \\
\bottomrule
\multicolumn{11}{l}{\rule{0pt}{1em}\rule{0pt}{2em}\textsuperscript{*}\makecell[l]{The Gaussian method employs a sample covariance matrix and includes four techniques (G, B, H, HB)\\ with multi-step residuals.}}\\
\end{tabular}


==> tab/VN525/trash/sam_crps_free.tex <==

\begin{tabular}[t]{>{\centering\arraybackslash}p{2.5cm}>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}>{\centering\arraybackslash}p{1cm}}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{9}{c}{\textbf{Base forecasts' sample approach}} \\
\cmidrule(l{0pt}r{0pt}){2-10}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{8}{c}{Gaussian frameworks: sample covariance matrix} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{4}{c}{Multi-step residuals} & \multicolumn{4}{c}{\makecell[c]{Overlapping and\\multi-step residuals}} \\
\multirow{-5}{*}{\parbox{2cm}{\centering\textbf{Reconciliation\\approach}}} & \multirow{-4}{*}{Bootstrap} & G & B & H & HB & G & B & H & HB\\
\midrule
\addlinespace[0.3em]
\multicolumn{10}{c}{\textbf{$\forall k \in \{12,6,4,3,2,1\}$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.970} & \textcolor{black}{0.970} & \textcolor{black}{0.971} & \textcolor{black}{0.971} & \textcolor{red}{1.002} & \textcolor{red}{1.066} & \textcolor{black}{0.971} & \textcolor{black}{0.971}\\
ct$(bu_{cs}, bu_{te})$ & \textcolor{red}{1.319} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.059} & \textcolor{red}{1.059} & \textcolor{red}{1.059} & \textcolor{red}{1.059}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.064} & \textcolor{black}{0.969} & \textcolor{black}{0.964} & \textcolor{black}{0.969} & \textcolor{black}{0.964} & \textcolor{red}{1.105} & \textcolor{red}{1.078} & \textcolor{red}{1.104} & \textcolor{red}{1.078}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.084} & \textcolor{black}{0.971} & \textcolor{black}{0.970} & \textcolor{black}{0.971} & \textcolor{black}{0.970} & \textcolor{black}{0.982} & \textcolor{black}{\textbf{0.982}} & \textcolor{black}{0.982} & \textcolor{black}{0.982}\\
oct$(wlsv)$ & \textcolor{black}{0.987} & \textcolor{black}{0.952} & \textcolor{black}{0.951} & \textcolor{black}{0.951} & \textcolor{black}{0.951} & \textcolor{black}{\textbf{0.953}} & \textcolor{red}{2.362} & \textcolor{black}{0.953} & \textcolor{black}{0.954}\\
oct$(bdshr)$ & \textcolor{black}{\textbf{0.976}} & \textcolor{black}{\textbf{0.949}} & \textcolor{black}{\textbf{0.947}} & \textcolor{blue}{\textbf{0.946}} & \textcolor{black}{\textbf{0.946}} & \textcolor{red}{1.040} & \textcolor{red}{57.782} & \textcolor{red}{1.013} & \textcolor{red}{1.009}\\
oct$_o(wlsv)$ & \textcolor{black}{0.988} & \textcolor{black}{0.951} & \textcolor{black}{0.950} & \textcolor{black}{0.950} & \textcolor{black}{0.950} & \textcolor{black}{0.987} & \textcolor{red}{2.496} & \textcolor{black}{\textbf{0.952}} & \textcolor{black}{\textbf{0.953}}\\
oct$_o(bdshr)$ & \textcolor{red}{1.060} & \textcolor{red}{1.051} & \textcolor{red}{1.034} & \textcolor{red}{1.036} & \textcolor{red}{1.029} & \textcolor{red}{1.877} & \textcolor{red}{64.627} & \textcolor{red}{1.029} & \textcolor{red}{1.026}\\
\addlinespace[0.3em]
\multicolumn{10}{c}{\textbf{$k = 1$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.972} & \textcolor{black}{0.972} & \textcolor{black}{0.972} & \textcolor{black}{0.972} & \textcolor{black}{0.976} & \textcolor{black}{0.976} & \textcolor{black}{0.976} & \textcolor{black}{0.977}\\
ct$(bu_{cs}, bu_{te})$ & \textcolor{red}{1.077} & \textcolor{black}{0.983} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.994} & \textcolor{black}{0.993} & \textcolor{black}{0.994} & \textcolor{black}{0.994}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{black}{0.980} & \textcolor{black}{0.968} & \textcolor{black}{0.968} & \textcolor{black}{0.968} & \textcolor{black}{0.968} & \textcolor{red}{1.033} & \textcolor{red}{1.036} & \textcolor{red}{1.033} & \textcolor{red}{1.036}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{black}{0.987} & \textcolor{black}{0.970} & \textcolor{black}{0.970} & \textcolor{black}{0.970} & \textcolor{black}{0.970} & \textcolor{black}{0.972} & \textcolor{black}{\textbf{0.974}} & \textcolor{black}{0.972} & \textcolor{black}{0.974}\\
oct$(wlsv)$ & \textcolor{black}{0.953} & \textcolor{black}{0.965} & \textcolor{black}{0.965} & \textcolor{black}{0.965} & \textcolor{black}{0.966} & \textcolor{black}{\textbf{0.967}} & \textcolor{red}{2.167} & \textcolor{black}{0.968} & \textcolor{black}{0.970}\\
oct$(bdshr)$ & \textcolor{blue}{\textbf{0.950}} & \textcolor{black}{\textbf{0.962}} & \textcolor{black}{\textbf{0.962}} & \textcolor{black}{\textbf{0.962}} & \textcolor{black}{\textbf{0.963}} & \textcolor{red}{1.002} & \textcolor{red}{60.461} & \textcolor{red}{1.002} & \textcolor{red}{1.009}\\
oct$_o(wlsv)$ & \textcolor{black}{0.954} & \textcolor{black}{0.964} & \textcolor{black}{0.964} & \textcolor{black}{0.965} & \textcolor{black}{0.965} & \textcolor{black}{0.995} & \textcolor{red}{2.276} & \textcolor{black}{\textbf{0.968}} & \textcolor{black}{\textbf{0.970}}\\
oct$_o(bdshr)$ & \textcolor{red}{1.005} & \textcolor{red}{1.020} & \textcolor{red}{1.017} & \textcolor{red}{1.019} & \textcolor{red}{1.018} & \textcolor{red}{1.754} & \textcolor{red}{65.650} & \textcolor{red}{1.014} & \textcolor{red}{1.019}\\
\addlinespace[0.3em]
\multicolumn{10}{c}{\textbf{$k = 3$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.971} & \textcolor{black}{0.971} & \textcolor{black}{0.972} & \textcolor{black}{0.973} & \textcolor{red}{1.065} & \textcolor{red}{1.285} & \textcolor{black}{0.969} & \textcolor{black}{0.969}\\
ct$(bu_{cs}, bu_{te})$ & \textcolor{red}{1.273} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.051} & \textcolor{red}{1.050} & \textcolor{red}{1.051} & \textcolor{red}{1.050}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.046} & \textcolor{black}{0.973} & \textcolor{black}{0.971} & \textcolor{black}{0.973} & \textcolor{black}{0.971} & \textcolor{red}{1.077} & \textcolor{red}{1.063} & \textcolor{red}{1.077} & \textcolor{red}{1.063}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.063} & \textcolor{black}{0.975} & \textcolor{black}{0.975} & \textcolor{black}{0.975} & \textcolor{black}{0.975} & \textcolor{black}{0.981} & \textcolor{black}{\textbf{0.981}} & \textcolor{black}{0.981} & \textcolor{black}{0.981}\\
oct$(wlsv)$ & \textcolor{black}{0.983} & \textcolor{black}{0.955} & \textcolor{black}{0.955} & \textcolor{black}{0.955} & \textcolor{black}{0.956} & \textcolor{black}{\textbf{0.953}} & \textcolor{red}{2.323} & \textcolor{black}{0.953} & \textcolor{black}{0.954}\\
oct$(bdshr)$ & \textcolor{black}{\textbf{0.973}} & \textcolor{black}{\textbf{0.953}} & \textcolor{black}{\textbf{0.951}} & \textcolor{blue}{\textbf{0.951}} & \textcolor{black}{\textbf{0.952}} & \textcolor{red}{1.014} & \textcolor{red}{63.627} & \textcolor{red}{1.004} & \textcolor{red}{1.004}\\
oct$_o(wlsv)$ & \textcolor{black}{0.984} & \textcolor{black}{0.954} & \textcolor{black}{0.954} & \textcolor{black}{0.954} & \textcolor{black}{0.955} & \textcolor{black}{0.983} & \textcolor{red}{2.450} & \textcolor{black}{\textbf{0.952}} & \textcolor{black}{\textbf{0.953}}\\
oct$_o(bdshr)$ & \textcolor{red}{1.046} & \textcolor{red}{1.038} & \textcolor{red}{1.030} & \textcolor{red}{1.031} & \textcolor{red}{1.029} & \textcolor{red}{1.814} & \textcolor{red}{72.720} & \textcolor{red}{1.019} & \textcolor{red}{1.019}\\
\addlinespace[0.3em]
\multicolumn{10}{c}{\textbf{$k = 12$}}\\
base & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{0.968} & \textcolor{black}{0.967} & \textcolor{black}{0.969} & \textcolor{black}{0.969} & \textcolor{black}{0.967} & \textcolor{black}{\textbf{0.965}} & \textcolor{black}{0.968} & \textcolor{black}{0.968}\\
ct$(bu_{cs}, bu_{te})$ & \textcolor{red}{1.675} & \textcolor{red}{1.038} & \textcolor{red}{1.037} & \textcolor{red}{1.037} & \textcolor{red}{1.038} & \textcolor{red}{1.138} & \textcolor{red}{1.138} & \textcolor{red}{1.138} & \textcolor{red}{1.138}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.174} & \textcolor{black}{0.965} & \textcolor{black}{0.955} & \textcolor{black}{0.965} & \textcolor{black}{0.955} & \textcolor{red}{1.211} & \textcolor{red}{1.138} & \textcolor{red}{1.211} & \textcolor{red}{1.138}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.214} & \textcolor{black}{0.967} & \textcolor{black}{0.965} & \textcolor{black}{0.967} & \textcolor{black}{0.965} & \textcolor{black}{0.993} & \textcolor{black}{0.991} & \textcolor{black}{0.993} & \textcolor{black}{0.991}\\
oct$(wlsv)$ & \textcolor{red}{1.026} & \textcolor{black}{0.935} & \textcolor{black}{0.934} & \textcolor{black}{0.932} & \textcolor{black}{0.932} & \textcolor{black}{\textbf{0.940}} & \textcolor{red}{2.616} & \textcolor{black}{0.938} & \textcolor{black}{0.939}\\
oct$(bdshr)$ & \textcolor{red}{1.006} & \textcolor{black}{0.934} & \textcolor{black}{\textbf{0.928}} & \textcolor{black}{\textbf{0.925}} & \textcolor{blue}{\textbf{0.924}} & \textcolor{red}{1.107} & \textcolor{red}{50.149} & \textcolor{red}{1.033} & \textcolor{red}{1.014}\\
oct$_o(wlsv)$ & \textcolor{red}{1.026} & \textcolor{black}{\textbf{0.933}} & \textcolor{black}{0.932} & \textcolor{black}{0.931} & \textcolor{black}{0.931} & \textcolor{black}{0.983} & \textcolor{red}{2.789} & \textcolor{black}{\textbf{0.937}} & \textcolor{black}{\textbf{0.938}}\\
oct$_o(bdshr)$ & \textcolor{red}{1.132} & \textcolor{red}{1.095} & \textcolor{red}{1.055} & \textcolor{red}{1.057} & \textcolor{red}{1.039} & \textcolor{red}{2.077} & \textcolor{red}{56.540} & \textcolor{red}{1.054} & \textcolor{red}{1.039}\\
\bottomrule
\end{tabular}


==> tab/VN525/trash/sam_crps_more.tex <==

\begin{tabular}[t]{c|>{}cccc>{}c|ccccc}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{10}{c}{\textbf{Base forecasts' sample approach}} \\
\cmidrule(l{0pt}r{0pt}){2-11}
\multicolumn{1}{c}{\makecell[c]{\bfseries Reconciliation\\\bfseries approach}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} \\
\multicolumn{1}{c}{} &  & G & B & H & \multicolumn{1}{c}{HB} &  & G & B & H & HB\\
\midrule
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$\forall k \in \{12,6,4,3,2,1\}$}} & \multicolumn{5}{c}{\textbf{$k = 1$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.971} & \textcolor{black}{0.971} & \textcolor{black}{0.973} & \textcolor{black}{0.973} & \textcolor{black}{1.000} & \textcolor{black}{0.972} & \textcolor{black}{0.972} & \textcolor{black}{0.972} & \textcolor{black}{0.972}\\
ct$(bu)$ & \textcolor{red}{1.321} & \textcolor{red}{1.011} & \textcolor{red}{1.011} & \textcolor{red}{1.011} & \textcolor{red}{1.011} & \textcolor{red}{1.077} & \textcolor{black}{0.983} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.982}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.057} & \textcolor{black}{0.974} & \textcolor{black}{0.969} & \textcolor{black}{0.974} & \textcolor{black}{0.969} & \textcolor{black}{0.976} & \textcolor{black}{0.963} & \textcolor{black}{0.962} & \textcolor{black}{0.963} & \textcolor{black}{0.962}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.082} & \textcolor{black}{0.977} & \textcolor{black}{0.976} & \textcolor{black}{0.977} & \textcolor{black}{0.976} & \textcolor{black}{0.986} & \textcolor{black}{0.965} & \textcolor{black}{0.965} & \textcolor{black}{0.965} & \textcolor{black}{0.965}\\
oct$(ols)$ & \textcolor{black}{0.989} & \textcolor{black}{0.989} & \textcolor{black}{0.989} & \textcolor{black}{0.987} & \textcolor{black}{0.987} & \textcolor{black}{0.982} & \textcolor{black}{0.986} & \textcolor{black}{0.988} & \textcolor{black}{0.986} & \textcolor{black}{0.989}\\
oct$(struc)$ & \textcolor{black}{0.982} & \textcolor{black}{0.962} & \textcolor{black}{0.961} & \textcolor{black}{0.961} & \textcolor{black}{0.959} & \textcolor{black}{0.970} & \textcolor{black}{0.963} & \textcolor{black}{0.963} & \textcolor{black}{0.963} & \textcolor{black}{0.963}\\
oct$(wlsv)$ & \textcolor{black}{0.987} & \textcolor{black}{0.959} & \textcolor{black}{0.959} & \textcolor{black}{0.958} & \textcolor{black}{0.957} & \textcolor{black}{0.952} & \textcolor{black}{0.957} & \textcolor{black}{0.957} & \textcolor{black}{0.957} & \textcolor{black}{0.957}\\
oct$(bdshr)$ & \textcolor{black}{\textbf{0.975}} & \textcolor{black}{\textbf{0.956}} & \textcolor{black}{\textbf{0.953}} & \textcolor{black}{\textbf{0.952}} & \textcolor{blue}{\textbf{0.951}} & \textcolor{blue}{\textbf{0.949}} & \textcolor{black}{\textbf{0.955}} & \textcolor{black}{\textbf{0.953}} & \textcolor{black}{\textbf{0.954}} & \textcolor{black}{\textbf{0.954}}\\
oct$_h(hbshr)$ &  &  &  & \textcolor{red}{1.016} & \textcolor{red}{1.018} &  &  &  & \textcolor{red}{1.004} & \textcolor{red}{1.009}\\
oct$_h(bshr)$ &  &  &  & \textcolor{red}{1.016} & \textcolor{red}{1.019} &  &  &  & \textcolor{red}{1.006} & \textcolor{red}{1.012}\\
oct$_h(hshr)$ &  &  &  & \textcolor{black}{0.990} & \textcolor{black}{0.991} &  &  &  & \textcolor{black}{0.979} & \textcolor{black}{0.979}\\
oct$_h(shr)$ &  &  &  & \textcolor{black}{0.970} & \textcolor{black}{0.970} &  &  &  & \textcolor{black}{0.976} & \textcolor{black}{0.974}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 2$}} & \multicolumn{5}{c}{\textbf{$k = 3$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.970} & \textcolor{black}{0.969} & \textcolor{black}{0.970} & \textcolor{black}{0.971} & \textcolor{black}{1.000} & \textcolor{black}{0.971} & \textcolor{black}{0.971} & \textcolor{black}{0.972} & \textcolor{black}{0.973}\\
ct$(bu)$ & \textcolor{red}{1.189} & \textcolor{black}{0.999} & \textcolor{black}{0.999} & \textcolor{black}{0.999} & \textcolor{black}{0.999} & \textcolor{red}{1.273} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.010}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.015} & \textcolor{black}{0.972} & \textcolor{black}{0.970} & \textcolor{black}{0.972} & \textcolor{black}{0.970} & \textcolor{red}{1.041} & \textcolor{black}{0.977} & \textcolor{black}{0.974} & \textcolor{black}{0.977} & \textcolor{black}{0.974}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.031} & \textcolor{black}{0.975} & \textcolor{black}{0.974} & \textcolor{black}{0.975} & \textcolor{black}{0.974} & \textcolor{red}{1.062} & \textcolor{black}{0.980} & \textcolor{black}{0.979} & \textcolor{black}{0.980} & \textcolor{black}{0.979}\\
oct$(ols)$ & \textcolor{black}{0.992} & \textcolor{black}{0.991} & \textcolor{black}{0.991} & \textcolor{black}{0.990} & \textcolor{black}{0.991} & \textcolor{black}{0.994} & \textcolor{black}{0.992} & \textcolor{black}{0.993} & \textcolor{black}{0.991} & \textcolor{black}{0.992}\\
oct$(struc)$ & \textcolor{black}{0.982} & \textcolor{black}{0.966} & \textcolor{black}{0.965} & \textcolor{black}{0.965} & \textcolor{black}{0.965} & \textcolor{black}{0.986} & \textcolor{black}{0.967} & \textcolor{black}{0.966} & \textcolor{black}{0.966} & \textcolor{black}{0.965}\\
oct$(wlsv)$ & \textcolor{black}{0.972} & \textcolor{black}{0.961} & \textcolor{black}{0.960} & \textcolor{black}{0.960} & \textcolor{black}{0.960} & \textcolor{black}{0.983} & \textcolor{black}{0.963} & \textcolor{black}{0.962} & \textcolor{black}{0.962} & \textcolor{black}{0.962}\\
oct$(bdshr)$ & \textcolor{black}{\textbf{0.964}} & \textcolor{black}{\textbf{0.958}} & \textcolor{black}{\textbf{0.957}} & \textcolor{black}{\textbf{0.956}} & \textcolor{blue}{\textbf{0.956}} & \textcolor{black}{\textbf{0.972}} & \textcolor{black}{\textbf{0.960}} & \textcolor{black}{\textbf{0.958}} & \textcolor{black}{\textbf{0.957}} & \textcolor{blue}{\textbf{0.957}}\\
oct$_h(hbshr)$ &  &  &  & \textcolor{red}{1.012} & \textcolor{red}{1.015} &  &  &  & \textcolor{red}{1.018} & \textcolor{red}{1.020}\\
oct$_h(bshr)$ &  &  &  & \textcolor{red}{1.013} & \textcolor{red}{1.017} &  &  &  & \textcolor{red}{1.018} & \textcolor{red}{1.022}\\
oct$_h(hshr)$ &  &  &  & \textcolor{black}{0.986} & \textcolor{black}{0.987} &  &  &  & \textcolor{black}{0.992} & \textcolor{black}{0.993}\\
oct$_h(shr)$ &  &  &  & \textcolor{black}{0.976} & \textcolor{black}{0.975} &  &  &  & \textcolor{black}{0.976} & \textcolor{black}{0.976}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 4$}} & \multicolumn{5}{c}{\textbf{$k = 6$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.973} & \textcolor{black}{0.973} & \textcolor{black}{0.974} & \textcolor{black}{0.975} & \textcolor{black}{1.000} & \textcolor{black}{0.976} & \textcolor{black}{0.976} & \textcolor{black}{0.978} & \textcolor{black}{0.978}\\
ct$(bu)$ & \textcolor{red}{1.340} & \textcolor{red}{1.016} & \textcolor{red}{1.015} & \textcolor{red}{1.015} & \textcolor{red}{1.015} & \textcolor{red}{1.450} & \textcolor{red}{1.023} & \textcolor{red}{1.023} & \textcolor{red}{1.023} & \textcolor{red}{1.023}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.061} & \textcolor{black}{0.978} & \textcolor{black}{0.973} & \textcolor{black}{0.978} & \textcolor{black}{0.973} & \textcolor{red}{1.094} & \textcolor{black}{0.978} & \textcolor{black}{0.972} & \textcolor{black}{0.978} & \textcolor{black}{0.972}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.087} & \textcolor{black}{0.982} & \textcolor{black}{0.980} & \textcolor{black}{0.982} & \textcolor{black}{0.980} & \textcolor{red}{1.127} & \textcolor{black}{0.982} & \textcolor{black}{0.981} & \textcolor{black}{0.982} & \textcolor{black}{0.981}\\
oct$(ols)$ & \textcolor{black}{0.993} & \textcolor{black}{0.991} & \textcolor{black}{0.992} & \textcolor{black}{0.990} & \textcolor{black}{0.990} & \textcolor{black}{0.989} & \textcolor{black}{0.989} & \textcolor{black}{0.989} & \textcolor{black}{0.987} & \textcolor{black}{0.986}\\
oct$(struc)$ & \textcolor{black}{0.986} & \textcolor{black}{0.965} & \textcolor{black}{0.964} & \textcolor{black}{0.964} & \textcolor{black}{0.963} & \textcolor{black}{0.986} & \textcolor{black}{0.961} & \textcolor{black}{0.960} & \textcolor{black}{0.959} & \textcolor{black}{0.957}\\
oct$(wlsv)$ & \textcolor{black}{0.990} & \textcolor{black}{0.962} & \textcolor{black}{0.961} & \textcolor{black}{0.961} & \textcolor{black}{0.960} & \textcolor{red}{1.001} & \textcolor{black}{0.960} & \textcolor{black}{0.959} & \textcolor{black}{0.958} & \textcolor{black}{0.957}\\
oct$(bdshr)$ & \textcolor{black}{\textbf{0.977}} & \textcolor{black}{\textbf{0.959}} & \textcolor{black}{\textbf{0.956}} & \textcolor{black}{\textbf{0.955}} & \textcolor{blue}{\textbf{0.954}} & \textcolor{black}{\textbf{0.985}} & \textcolor{black}{\textbf{0.956}} & \textcolor{black}{\textbf{0.953}} & \textcolor{black}{\textbf{0.950}} & \textcolor{blue}{\textbf{0.948}}\\
oct$_h(hbshr)$ &  &  &  & \textcolor{red}{1.019} & \textcolor{red}{1.021} &  &  &  & \textcolor{red}{1.022} & \textcolor{red}{1.022}\\
oct$_h(bshr)$ &  &  &  & \textcolor{red}{1.019} & \textcolor{red}{1.022} &  &  &  & \textcolor{red}{1.020} & \textcolor{red}{1.022}\\
oct$_h(hshr)$ &  &  &  & \textcolor{black}{0.994} & \textcolor{black}{0.995} &  &  &  & \textcolor{black}{0.996} & \textcolor{black}{0.997}\\
oct$_h(shr)$ &  &  &  & \textcolor{black}{0.973} & \textcolor{black}{0.973} &  &  &  & \textcolor{black}{0.967} & \textcolor{black}{0.967}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 12$}} & \multicolumn{5}{c}{}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.968} & \textcolor{black}{0.967} & \textcolor{black}{0.969} & \textcolor{black}{0.969} &  &  &  &  & \\
ct$(bu)$ & \textcolor{red}{1.675} & \textcolor{red}{1.038} & \textcolor{red}{1.037} & \textcolor{red}{1.037} & \textcolor{red}{1.038} &  &  &  &  & \\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.163} & \textcolor{black}{0.977} & \textcolor{black}{0.965} & \textcolor{black}{0.977} & \textcolor{black}{0.965} &  &  &  &  & \\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.212} & \textcolor{black}{0.980} & \textcolor{black}{0.976} & \textcolor{black}{0.980} & \textcolor{black}{0.976} &  &  &  &  & \\
oct$(ols)$ & \textcolor{black}{\textbf{0.982}} & \textcolor{black}{0.982} & \textcolor{black}{0.983} & \textcolor{black}{0.980} & \textcolor{black}{0.975} &  &  &  &  & \\
oct$(struc)$ & \textcolor{black}{0.982} & \textcolor{black}{0.951} & \textcolor{black}{0.949} & \textcolor{black}{0.947} & \textcolor{black}{0.943} &  &  &  &  & \\
oct$(wlsv)$ & \textcolor{red}{1.025} & \textcolor{black}{0.954} & \textcolor{black}{0.953} & \textcolor{black}{0.949} & \textcolor{black}{0.947} &  &  &  &  & \\
oct$(bdshr)$ & \textcolor{red}{1.002} & \textcolor{black}{\textbf{0.950}} & \textcolor{black}{\textbf{0.944}} & \textcolor{black}{\textbf{0.939}} & \textcolor{blue}{\textbf{0.935}} &  &  &  &  & \\
oct$_h(hbshr)$ &  &  &  & \textcolor{red}{1.024} & \textcolor{red}{1.021} &  &  &  &  & \\
oct$_h(bshr)$ &  &  &  & \textcolor{red}{1.021} & \textcolor{red}{1.019} &  &  &  &  & \\
oct$_h(hshr)$ &  &  &  & \textcolor{black}{0.996} & \textcolor{black}{0.997} &  &  &  &  & \\
oct$_h(shr)$ &  &  &  & \textcolor{black}{0.952} & \textcolor{black}{0.952} &  &  &  &  & \\
\bottomrule
\multicolumn{11}{l}{\rule{0pt}{1em}\rule{0pt}{1.75em}\makecell[l]{$^\ast$The Gaussian method employs a sample covariance matrix and includes four techniques (G, B, H, HB)\\ with multi-step residuals.}}\\
\end{tabular}


==> tab/VN525/trash/sam_crps_old.tex <==

\begin{tabular}[t]{>{\centering\arraybackslash}p{2.5cm}>{\centering\arraybackslash}p{1.5cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{9}{c}{\textbf{Base forecasts' sample approach}} \\
\cmidrule(l{0pt}r{0pt}){2-10}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{8}{c}{Gaussian frameworks: sample covariance matrix} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{4}{c}{Multi-step residuals} & \multicolumn{4}{c}{\makecell[c]{Overlapping and\\multi-step residuals}} \\
\multirow{-5}{*}{\parbox{2cm}{\centering\textbf{Reconciliation\\approach}}} & \multirow{-4}{*}{Bootstrap} & G & B & H & HB & G & B & H & HB\\
\midrule
\addlinespace[0.3em]
\multicolumn{10}{c}{\textbf{$\forall k \in \{12,6,4,3,2,1\}$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.970} & \textcolor{black}{0.970} & \textcolor{black}{0.971} & \textcolor{black}{0.971} & \textcolor{red}{1.002} & \textcolor{red}{1.066} & \textcolor{black}{\textbf{0.971}} & \textcolor{black}{\textbf{0.971}}\\
ct$(bu_{cs}, bu_{te})$ & \textcolor{red}{1.319} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.059} & \textcolor{red}{1.059} & \textcolor{red}{1.059} & \textcolor{red}{1.059}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.057} & \textcolor{black}{0.972} & \textcolor{black}{0.967} & \textcolor{black}{0.972} & \textcolor{black}{0.967} & \textcolor{red}{1.109} & \textcolor{red}{1.079} & \textcolor{red}{1.109} & \textcolor{red}{1.079}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.083} & \textcolor{black}{0.975} & \textcolor{black}{0.974} & \textcolor{black}{0.975} & \textcolor{black}{0.974} & \textcolor{red}{1.002} & \textcolor{red}{\textbf{1.001}} & \textcolor{red}{1.002} & \textcolor{red}{1.002}\\
oct$(wlsv)$ & \textcolor{black}{0.986} & \textcolor{black}{0.958} & \textcolor{black}{0.957} & \textcolor{black}{0.956} & \textcolor{black}{0.955} & \textcolor{black}{\textbf{0.977}} & \textcolor{red}{2.386} & \textcolor{black}{0.975} & \textcolor{black}{0.974}\\
oct$(bdshr)$ & \textcolor{black}{\textbf{0.974}} & \textcolor{black}{\textbf{0.955}} & \textcolor{black}{\textbf{0.952}} & \textcolor{black}{\textbf{0.950}} & \textcolor{blue}{\textbf{0.949}} & \textcolor{red}{1.046} & \textcolor{red}{59.818} & \textcolor{red}{1.017} & \textcolor{red}{1.010}\\
oct$_o(wlsv)$ & \textcolor{black}{0.987} & \textcolor{black}{0.957} & \textcolor{black}{0.956} & \textcolor{black}{0.955} & \textcolor{black}{0.954} & \textcolor{red}{1.021} & \textcolor{red}{2.516} & \textcolor{black}{0.974} & \textcolor{black}{0.974}\\
oct$_o(bdshr)$ & \textcolor{red}{1.038} & \textcolor{red}{1.039} & \textcolor{red}{1.016} & \textcolor{red}{1.019} & \textcolor{red}{1.007} & \textcolor{red}{1.909} & \textcolor{red}{63.888} & \textcolor{red}{1.025} & \textcolor{red}{1.018}\\
\addlinespace[0.3em]
\multicolumn{10}{c}{\textbf{$k = 1$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.972} & \textcolor{black}{0.972} & \textcolor{black}{0.972} & \textcolor{black}{0.972} & \textcolor{black}{0.976} & \textcolor{black}{0.976} & \textcolor{black}{0.976} & \textcolor{black}{0.977}\\
ct$(bu_{cs}, bu_{te})$ & \textcolor{red}{1.077} & \textcolor{black}{0.983} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.994} & \textcolor{black}{0.993} & \textcolor{black}{0.994} & \textcolor{black}{0.994}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{black}{0.976} & \textcolor{black}{0.963} & \textcolor{black}{0.962} & \textcolor{black}{0.963} & \textcolor{black}{0.962} & \textcolor{red}{1.015} & \textcolor{red}{1.010} & \textcolor{red}{1.015} & \textcolor{red}{1.010}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{black}{0.986} & \textcolor{black}{0.965} & \textcolor{black}{0.965} & \textcolor{black}{0.965} & \textcolor{black}{0.965} & \textcolor{black}{0.965} & \textcolor{black}{\textbf{0.965}} & \textcolor{black}{0.965} & \textcolor{black}{0.965}\\
oct$(wlsv)$ & \textcolor{black}{0.952} & \textcolor{black}{0.957} & \textcolor{black}{0.957} & \textcolor{black}{0.957} & \textcolor{black}{0.957} & \textcolor{black}{\textbf{0.952}} & \textcolor{red}{1.980} & \textcolor{black}{0.952} & \textcolor{black}{0.953}\\
oct$(bdshr)$ & \textcolor{blue}{\textbf{0.949}} & \textcolor{black}{\textbf{0.955}} & \textcolor{black}{\textbf{0.953}} & \textcolor{black}{\textbf{0.954}} & \textcolor{black}{\textbf{0.954}} & \textcolor{black}{0.979} & \textcolor{red}{39.336} & \textcolor{black}{0.976} & \textcolor{black}{0.976}\\
oct$_o(wlsv)$ & \textcolor{black}{0.953} & \textcolor{black}{0.957} & \textcolor{black}{0.956} & \textcolor{black}{0.957} & \textcolor{black}{0.957} & \textcolor{black}{0.980} & \textcolor{red}{2.058} & \textcolor{black}{\textbf{0.952}} & \textcolor{black}{\textbf{0.953}}\\
oct$_o(bdshr)$ & \textcolor{black}{0.990} & \textcolor{black}{0.999} & \textcolor{black}{0.993} & \textcolor{black}{0.996} & \textcolor{black}{0.992} & \textcolor{red}{1.524} & \textcolor{red}{41.933} & \textcolor{black}{0.983} & \textcolor{black}{0.982}\\
\addlinespace[0.3em]
\multicolumn{10}{c}{\textbf{$k = 3$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.971} & \textcolor{black}{0.971} & \textcolor{black}{0.972} & \textcolor{black}{0.973} & \textcolor{red}{1.065} & \textcolor{red}{1.285} & \textcolor{black}{\textbf{0.969}} & \textcolor{black}{\textbf{0.969}}\\
ct$(bu_{cs}, bu_{te})$ & \textcolor{red}{1.273} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.010} & \textcolor{red}{1.051} & \textcolor{red}{1.050} & \textcolor{red}{1.051} & \textcolor{red}{1.050}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.041} & \textcolor{black}{0.977} & \textcolor{black}{0.974} & \textcolor{black}{0.977} & \textcolor{black}{0.974} & \textcolor{red}{1.086} & \textcolor{red}{1.068} & \textcolor{red}{1.086} & \textcolor{red}{1.068}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.062} & \textcolor{black}{0.980} & \textcolor{black}{0.979} & \textcolor{black}{0.980} & \textcolor{black}{0.979} & \textcolor{red}{1.000} & \textcolor{black}{\textbf{1.000}} & \textcolor{red}{1.000} & \textcolor{black}{1.000}\\
oct$(wlsv)$ & \textcolor{black}{0.983} & \textcolor{black}{0.963} & \textcolor{black}{0.962} & \textcolor{black}{0.962} & \textcolor{black}{0.962} & \textcolor{black}{\textbf{0.976}} & \textcolor{red}{2.335} & \textcolor{black}{0.975} & \textcolor{black}{0.975}\\
oct$(bdshr)$ & \textcolor{black}{\textbf{0.972}} & \textcolor{black}{\textbf{0.960}} & \textcolor{black}{\textbf{0.958}} & \textcolor{black}{\textbf{0.957}} & \textcolor{blue}{\textbf{0.957}} & \textcolor{red}{1.026} & \textcolor{red}{58.332} & \textcolor{red}{1.011} & \textcolor{red}{1.007}\\
oct$_o(wlsv)$ & \textcolor{black}{0.984} & \textcolor{black}{0.962} & \textcolor{black}{0.962} & \textcolor{black}{0.961} & \textcolor{black}{0.961} & \textcolor{red}{1.016} & \textcolor{red}{2.458} & \textcolor{black}{0.974} & \textcolor{black}{0.974}\\
oct$_o(bdshr)$ & \textcolor{red}{1.031} & \textcolor{red}{1.031} & \textcolor{red}{1.017} & \textcolor{red}{1.019} & \textcolor{red}{1.011} & \textcolor{red}{1.824} & \textcolor{red}{62.293} & \textcolor{red}{1.019} & \textcolor{red}{1.015}\\
\addlinespace[0.3em]
\multicolumn{10}{c}{\textbf{$k = 12$}}\\
base & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{0.968} & \textcolor{black}{0.967} & \textcolor{black}{0.969} & \textcolor{black}{0.969} & \textcolor{black}{\textbf{0.967}} & \textcolor{black}{\textbf{0.965}} & \textcolor{black}{\textbf{0.968}} & \textcolor{black}{\textbf{0.968}}\\
ct$(bu_{cs}, bu_{te})$ & \textcolor{red}{1.675} & \textcolor{red}{1.038} & \textcolor{red}{1.037} & \textcolor{red}{1.037} & \textcolor{red}{1.038} & \textcolor{red}{1.138} & \textcolor{red}{1.138} & \textcolor{red}{1.138} & \textcolor{red}{1.138}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.163} & \textcolor{black}{0.977} & \textcolor{black}{0.965} & \textcolor{black}{0.977} & \textcolor{black}{0.965} & \textcolor{red}{1.238} & \textcolor{red}{1.165} & \textcolor{red}{1.237} & \textcolor{red}{1.165}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.212} & \textcolor{black}{0.980} & \textcolor{black}{0.976} & \textcolor{black}{0.980} & \textcolor{black}{0.976} & \textcolor{red}{1.043} & \textcolor{red}{1.040} & \textcolor{red}{1.043} & \textcolor{red}{1.041}\\
oct$(wlsv)$ & \textcolor{red}{1.025} & \textcolor{black}{0.954} & \textcolor{black}{0.953} & \textcolor{black}{0.949} & \textcolor{black}{0.947} & \textcolor{red}{1.002} & \textcolor{red}{2.937} & \textcolor{black}{0.997} & \textcolor{black}{0.996}\\
oct$(bdshr)$ & \textcolor{red}{1.002} & \textcolor{black}{\textbf{0.950}} & \textcolor{black}{\textbf{0.944}} & \textcolor{black}{\textbf{0.939}} & \textcolor{blue}{\textbf{0.935}} & \textcolor{red}{1.140} & \textcolor{red}{93.280} & \textcolor{red}{1.067} & \textcolor{red}{1.048}\\
oct$_o(wlsv)$ & \textcolor{red}{1.025} & \textcolor{black}{0.952} & \textcolor{black}{0.951} & \textcolor{black}{0.948} & \textcolor{black}{0.945} & \textcolor{red}{1.070} & \textcolor{red}{3.147} & \textcolor{black}{0.996} & \textcolor{black}{0.995}\\
oct$_o(bdshr)$ & \textcolor{red}{1.097} & \textcolor{red}{1.088} & \textcolor{red}{1.040} & \textcolor{red}{1.044} & \textcolor{red}{1.018} & \textcolor{red}{2.505} & \textcolor{red}{99.829} & \textcolor{red}{1.075} & \textcolor{red}{1.060}\\
\bottomrule
\end{tabular}


==> tab/VN525/trash/sam_es.tex <==

\begin{tabular}[t]{c|>{}cccc>{}c|ccccc}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{10}{c}{\textbf{Base forecasts' sample approach}} \\
\cmidrule(l{0pt}r{0pt}){2-11}
\multicolumn{1}{c}{\makecell[c]{\bfseries Reconciliation\\\bfseries approach}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} \\
\multicolumn{1}{c}{} &  & G & B & H & \multicolumn{1}{c}{HB} &  & G & B & H & HB\\
\midrule
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$\forall k \in \{12,6,4,3,2,1\}$}} & \multicolumn{5}{c}{\textbf{$k = 1$}}\\
base & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{0.956} & \textcolor{black}{0.955} & \textcolor{black}{0.958} & \textcolor{black}{0.951} & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{0.952} & \textcolor{black}{0.950} & \textcolor{black}{0.952} & \textcolor{black}{0.950}\\
ct$(bu)$ & \textcolor{red}{2.427} & \textcolor{black}{0.983} & \textcolor{black}{0.983} & \textcolor{black}{0.983} & \textcolor{black}{0.983} & \textcolor{red}{1.759} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.982}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.243} & \textcolor{black}{\textbf{0.886}} & \textcolor{blue}{\textbf{0.879}} & \textcolor{black}{\textbf{0.886}} & \textcolor{black}{\textbf{0.879}} & \textcolor{red}{1.098} & \textcolor{black}{\textbf{0.929}} & \textcolor{black}{\textbf{0.928}} & \textcolor{black}{\textbf{0.930}} & \textcolor{blue}{\textbf{0.927}}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.348} & \textcolor{black}{0.904} & \textcolor{black}{0.901} & \textcolor{black}{0.905} & \textcolor{black}{0.901} & \textcolor{red}{1.151} & \textcolor{black}{0.940} & \textcolor{black}{0.939} & \textcolor{black}{0.940} & \textcolor{black}{0.938}\\
oct$(wlsv)$ & \textcolor{red}{1.132} & \textcolor{black}{0.933} & \textcolor{black}{0.929} & \textcolor{black}{0.931} & \textcolor{black}{0.927} & \textcolor{red}{1.050} & \textcolor{black}{0.951} & \textcolor{black}{0.949} & \textcolor{black}{0.950} & \textcolor{black}{0.949}\\
oct$(bdshr)$ & \textcolor{red}{1.047} & \textcolor{black}{0.904} & \textcolor{black}{0.897} & \textcolor{black}{0.897} & \textcolor{black}{0.891} & \textcolor{red}{1.009} & \textcolor{black}{0.936} & \textcolor{black}{0.933} & \textcolor{black}{0.934} & \textcolor{black}{0.931}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 2$}} & \multicolumn{5}{c}{\textbf{$k = 3$}}\\
base & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{0.958} & \textcolor{black}{0.954} & \textcolor{black}{0.956} & \textcolor{black}{0.953} & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{0.961} & \textcolor{black}{0.958} & \textcolor{black}{0.960} & \textcolor{black}{0.955}\\
ct$(bu)$ & \textcolor{red}{2.176} & \textcolor{red}{1.001} & \textcolor{red}{1.001} & \textcolor{red}{1.001} & \textcolor{red}{1.001} & \textcolor{red}{2.428} & \textcolor{black}{0.998} & \textcolor{black}{0.997} & \textcolor{black}{0.997} & \textcolor{black}{0.997}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.192} & \textcolor{black}{\textbf{0.927}} & \textcolor{blue}{\textbf{0.921}} & \textcolor{black}{\textbf{0.927}} & \textcolor{black}{\textbf{0.921}} & \textcolor{red}{1.245} & \textcolor{black}{\textbf{0.911}} & \textcolor{blue}{\textbf{0.904}} & \textcolor{black}{\textbf{0.911}} & \textcolor{black}{\textbf{0.904}}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.275} & \textcolor{black}{0.942} & \textcolor{black}{0.939} & \textcolor{black}{0.942} & \textcolor{black}{0.939} & \textcolor{red}{1.348} & \textcolor{black}{0.927} & \textcolor{black}{0.924} & \textcolor{black}{0.928} & \textcolor{black}{0.924}\\
oct$(wlsv)$ & \textcolor{red}{1.110} & \textcolor{black}{0.960} & \textcolor{black}{0.958} & \textcolor{black}{0.958} & \textcolor{black}{0.955} & \textcolor{red}{1.142} & \textcolor{black}{0.953} & \textcolor{black}{0.949} & \textcolor{black}{0.951} & \textcolor{black}{0.946}\\
oct$(bdshr)$ & \textcolor{red}{1.045} & \textcolor{black}{0.938} & \textcolor{black}{0.933} & \textcolor{black}{0.933} & \textcolor{black}{0.929} & \textcolor{red}{1.060} & \textcolor{black}{0.926} & \textcolor{black}{0.920} & \textcolor{black}{0.921} & \textcolor{black}{0.915}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 4$}} & \multicolumn{5}{c}{\textbf{$k = 6$}}\\
base & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{0.960} & \textcolor{black}{0.960} & \textcolor{black}{0.962} & \textcolor{black}{0.956} & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{0.961} & \textcolor{black}{0.959} & \textcolor{black}{0.964} & \textcolor{black}{0.956}\\
ct$(bu)$ & \textcolor{red}{2.585} & \textcolor{black}{0.996} & \textcolor{black}{0.996} & \textcolor{black}{0.995} & \textcolor{black}{0.996} & \textcolor{red}{2.849} & \textcolor{red}{1.004} & \textcolor{red}{1.003} & \textcolor{red}{1.003} & \textcolor{red}{1.004}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.277} & \textcolor{black}{\textbf{0.898}} & \textcolor{blue}{\textbf{0.890}} & \textcolor{black}{\textbf{0.899}} & \textcolor{black}{\textbf{0.891}} & \textcolor{red}{1.339} & \textcolor{black}{\textbf{0.882}} & \textcolor{blue}{\textbf{0.873}} & \textcolor{black}{\textbf{0.883}} & \textcolor{black}{\textbf{0.874}}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.392} & \textcolor{black}{0.917} & \textcolor{black}{0.911} & \textcolor{black}{0.917} & \textcolor{black}{0.913} & \textcolor{red}{1.473} & \textcolor{black}{0.905} & \textcolor{black}{0.901} & \textcolor{black}{0.906} & \textcolor{black}{0.901}\\
oct$(wlsv)$ & \textcolor{red}{1.157} & \textcolor{black}{0.947} & \textcolor{black}{0.943} & \textcolor{black}{0.945} & \textcolor{black}{0.939} & \textcolor{red}{1.192} & \textcolor{black}{0.942} & \textcolor{black}{0.937} & \textcolor{black}{0.941} & \textcolor{black}{0.934}\\
oct$(bdshr)$ & \textcolor{red}{1.065} & \textcolor{black}{0.917} & \textcolor{black}{0.909} & \textcolor{black}{0.910} & \textcolor{black}{0.903} & \textcolor{red}{1.084} & \textcolor{black}{0.907} & \textcolor{black}{0.897} & \textcolor{black}{0.898} & \textcolor{black}{0.890}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 12$}} & \multicolumn{5}{c}{}\\
base & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{0.942} & \textcolor{black}{0.947} & \textcolor{black}{0.951} & \textcolor{black}{0.937} &  &  &  &  & \\
ct$(bu)$ & \textcolor{red}{2.990} & \textcolor{black}{0.922} & \textcolor{black}{0.921} & \textcolor{black}{0.923} & \textcolor{black}{0.923} &  &  &  &  & \\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.326} & \textcolor{black}{\textbf{0.779}} & \textcolor{black}{\textbf{0.767}} & \textcolor{black}{\textbf{0.777}} & \textcolor{blue}{\textbf{0.766}} &  &  &  &  & \\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.477} & \textcolor{black}{0.804} & \textcolor{black}{0.800} & \textcolor{black}{0.805} & \textcolor{black}{0.799} &  &  &  &  & \\
oct$(wlsv)$ & \textcolor{red}{1.149} & \textcolor{black}{0.851} & \textcolor{black}{0.845} & \textcolor{black}{0.847} & \textcolor{black}{0.840} &  &  &  &  & \\
oct$(bdshr)$ & \textcolor{red}{1.021} & \textcolor{black}{0.808} & \textcolor{black}{0.796} & \textcolor{black}{0.796} & \textcolor{black}{0.787} &  &  &  &  & \\
\bottomrule
\multicolumn{11}{l}{\rule{0pt}{1em}\rule{0pt}{2em}\textsuperscript{*}\makecell[l]{The Gaussian method employs a sample covariance matrix and includes four techniques (G, B, H, HB)\\ with multi-step residuals.}}\\
\end{tabular}


==> tab/VN525/trash/sam_es_more.tex <==

\begin{tabular}[t]{c|>{}cccc>{}c|ccccc}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{10}{c}{\textbf{Base forecasts' sample approach}} \\
\cmidrule(l{0pt}r{0pt}){2-11}
\multicolumn{1}{c}{\makecell[c]{\bfseries Reconciliation\\\bfseries approach}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} \\
\multicolumn{1}{c}{} &  & G & B & H & \multicolumn{1}{c}{HB} &  & G & B & H & HB\\
\midrule
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$\forall k \in \{12,6,4,3,2,1\}$}} & \multicolumn{5}{c}{\textbf{$k = 1$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.956} & \textcolor{black}{0.955} & \textcolor{black}{0.958} & \textcolor{black}{0.951} & \textcolor{black}{1.000} & \textcolor{black}{0.952} & \textcolor{black}{0.950} & \textcolor{black}{0.952} & \textcolor{black}{0.950}\\
ct$(bu)$ & \textcolor{red}{2.427} & \textcolor{black}{0.983} & \textcolor{black}{0.983} & \textcolor{black}{0.983} & \textcolor{black}{0.983} & \textcolor{red}{1.759} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.982}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.243} & \textcolor{black}{\textbf{0.886}} & \textcolor{black}{\textbf{0.879}} & \textcolor{black}{0.886} & \textcolor{black}{0.879} & \textcolor{red}{1.098} & \textcolor{black}{\textbf{0.929}} & \textcolor{black}{\textbf{0.928}} & \textcolor{black}{0.930} & \textcolor{black}{0.927}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.348} & \textcolor{black}{0.904} & \textcolor{black}{0.901} & \textcolor{black}{0.905} & \textcolor{black}{0.901} & \textcolor{red}{1.151} & \textcolor{black}{0.940} & \textcolor{black}{0.939} & \textcolor{black}{0.940} & \textcolor{black}{0.938}\\
oct$(ols)$ & \textcolor{black}{\textbf{0.955}} & \textcolor{black}{0.893} & \textcolor{black}{0.891} & \textcolor{black}{0.893} & \textcolor{black}{0.888} & \textcolor{black}{\textbf{0.975}} & \textcolor{black}{0.937} & \textcolor{black}{0.936} & \textcolor{black}{0.936} & \textcolor{black}{0.935}\\
oct$(struc)$ & \textcolor{red}{1.085} & \textcolor{black}{0.917} & \textcolor{black}{0.915} & \textcolor{black}{0.916} & \textcolor{black}{0.912} & \textcolor{red}{1.027} & \textcolor{black}{0.943} & \textcolor{black}{0.942} & \textcolor{black}{0.943} & \textcolor{black}{0.942}\\
oct$(wlsv)$ & \textcolor{red}{1.132} & \textcolor{black}{0.933} & \textcolor{black}{0.929} & \textcolor{black}{0.931} & \textcolor{black}{0.927} & \textcolor{red}{1.050} & \textcolor{black}{0.951} & \textcolor{black}{0.949} & \textcolor{black}{0.950} & \textcolor{black}{0.949}\\
oct$(bdshr)$ & \textcolor{red}{1.047} & \textcolor{black}{0.904} & \textcolor{black}{0.897} & \textcolor{black}{0.897} & \textcolor{black}{0.891} & \textcolor{red}{1.009} & \textcolor{black}{0.936} & \textcolor{black}{0.933} & \textcolor{black}{0.934} & \textcolor{black}{0.931}\\
oct$_h(hbshr)$ &  &  &  & \textcolor{black}{0.888} & \textcolor{black}{0.884} &  &  &  & \textcolor{black}{0.937} & \textcolor{black}{0.935}\\
oct$_h(bshr)$ &  &  &  & \textcolor{black}{\textbf{0.863}} & \textcolor{blue}{\textbf{0.860}} &  &  &  & \textcolor{black}{0.925} & \textcolor{black}{0.923}\\
oct$_h(hshr)$ &  &  &  & \textcolor{black}{0.935} & \textcolor{black}{0.927} &  &  &  & \textcolor{black}{0.952} & \textcolor{black}{0.950}\\
oct$_h(shr)$ &  &  &  & \textcolor{black}{0.875} & \textcolor{black}{0.864} &  &  &  & \textcolor{black}{\textbf{0.921}} & \textcolor{blue}{\textbf{0.916}}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 2$}} & \multicolumn{5}{c}{\textbf{$k = 3$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.958} & \textcolor{black}{0.954} & \textcolor{black}{0.956} & \textcolor{black}{0.953} & \textcolor{black}{1.000} & \textcolor{black}{0.961} & \textcolor{black}{0.958} & \textcolor{black}{0.960} & \textcolor{black}{0.955}\\
ct$(bu)$ & \textcolor{red}{2.176} & \textcolor{red}{1.001} & \textcolor{red}{1.001} & \textcolor{red}{1.001} & \textcolor{red}{1.001} & \textcolor{red}{2.428} & \textcolor{black}{0.998} & \textcolor{black}{0.997} & \textcolor{black}{0.997} & \textcolor{black}{0.997}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.192} & \textcolor{black}{\textbf{0.927}} & \textcolor{black}{\textbf{0.921}} & \textcolor{black}{0.927} & \textcolor{black}{0.921} & \textcolor{red}{1.245} & \textcolor{black}{\textbf{0.911}} & \textcolor{black}{\textbf{0.904}} & \textcolor{black}{0.911} & \textcolor{black}{0.904}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.275} & \textcolor{black}{0.942} & \textcolor{black}{0.939} & \textcolor{black}{0.942} & \textcolor{black}{0.939} & \textcolor{red}{1.348} & \textcolor{black}{0.927} & \textcolor{black}{0.924} & \textcolor{black}{0.928} & \textcolor{black}{0.924}\\
oct$(ols)$ & \textcolor{black}{\textbf{0.985}} & \textcolor{black}{0.935} & \textcolor{black}{0.932} & \textcolor{black}{0.934} & \textcolor{black}{0.930} & \textcolor{black}{\textbf{0.976}} & \textcolor{black}{0.918} & \textcolor{black}{0.915} & \textcolor{black}{0.917} & \textcolor{black}{0.912}\\
oct$(struc)$ & \textcolor{red}{1.075} & \textcolor{black}{0.949} & \textcolor{black}{0.947} & \textcolor{black}{0.948} & \textcolor{black}{0.944} & \textcolor{red}{1.096} & \textcolor{black}{0.939} & \textcolor{black}{0.936} & \textcolor{black}{0.938} & \textcolor{black}{0.933}\\
oct$(wlsv)$ & \textcolor{red}{1.110} & \textcolor{black}{0.960} & \textcolor{black}{0.958} & \textcolor{black}{0.958} & \textcolor{black}{0.955} & \textcolor{red}{1.142} & \textcolor{black}{0.953} & \textcolor{black}{0.949} & \textcolor{black}{0.951} & \textcolor{black}{0.946}\\
oct$(bdshr)$ & \textcolor{red}{1.045} & \textcolor{black}{0.938} & \textcolor{black}{0.933} & \textcolor{black}{0.933} & \textcolor{black}{0.929} & \textcolor{red}{1.060} & \textcolor{black}{0.926} & \textcolor{black}{0.920} & \textcolor{black}{0.921} & \textcolor{black}{0.915}\\
oct$_h(hbshr)$ &  &  &  & \textcolor{black}{0.933} & \textcolor{black}{0.928} &  &  &  & \textcolor{black}{0.915} & \textcolor{black}{0.909}\\
oct$_h(bshr)$ &  &  &  & \textcolor{black}{0.913} & \textcolor{black}{0.908} &  &  &  & \textcolor{black}{\textbf{0.892}} & \textcolor{blue}{\textbf{0.887}}\\
oct$_h(hshr)$ &  &  &  & \textcolor{black}{0.963} & \textcolor{black}{0.956} &  &  &  & \textcolor{black}{0.956} & \textcolor{black}{0.949}\\
oct$_h(shr)$ &  &  &  & \textcolor{black}{\textbf{0.913}} & \textcolor{blue}{\textbf{0.904}} &  &  &  & \textcolor{black}{0.900} & \textcolor{black}{0.890}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 4$}} & \multicolumn{5}{c}{\textbf{$k = 6$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.960} & \textcolor{black}{0.960} & \textcolor{black}{0.962} & \textcolor{black}{0.956} & \textcolor{black}{1.000} & \textcolor{black}{0.961} & \textcolor{black}{0.959} & \textcolor{black}{0.964} & \textcolor{black}{0.956}\\
ct$(bu)$ & \textcolor{red}{2.585} & \textcolor{black}{0.996} & \textcolor{black}{0.996} & \textcolor{black}{0.995} & \textcolor{black}{0.996} & \textcolor{red}{2.849} & \textcolor{red}{1.004} & \textcolor{red}{1.003} & \textcolor{red}{1.003} & \textcolor{red}{1.004}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.277} & \textcolor{black}{\textbf{0.898}} & \textcolor{black}{\textbf{0.890}} & \textcolor{black}{0.899} & \textcolor{black}{0.891} & \textcolor{red}{1.339} & \textcolor{black}{\textbf{0.882}} & \textcolor{black}{\textbf{0.873}} & \textcolor{black}{0.883} & \textcolor{black}{0.874}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.392} & \textcolor{black}{0.917} & \textcolor{black}{0.911} & \textcolor{black}{0.917} & \textcolor{black}{0.913} & \textcolor{red}{1.473} & \textcolor{black}{0.905} & \textcolor{black}{0.901} & \textcolor{black}{0.906} & \textcolor{black}{0.901}\\
oct$(ols)$ & \textcolor{black}{\textbf{0.966}} & \textcolor{black}{0.905} & \textcolor{black}{0.902} & \textcolor{black}{0.904} & \textcolor{black}{0.899} & \textcolor{black}{\textbf{0.962}} & \textcolor{black}{0.889} & \textcolor{black}{0.887} & \textcolor{black}{0.890} & \textcolor{black}{0.885}\\
oct$(struc)$ & \textcolor{red}{1.106} & \textcolor{black}{0.930} & \textcolor{black}{0.927} & \textcolor{black}{0.928} & \textcolor{black}{0.924} & \textcolor{red}{1.132} & \textcolor{black}{0.923} & \textcolor{black}{0.919} & \textcolor{black}{0.922} & \textcolor{black}{0.916}\\
oct$(wlsv)$ & \textcolor{red}{1.157} & \textcolor{black}{0.947} & \textcolor{black}{0.943} & \textcolor{black}{0.945} & \textcolor{black}{0.939} & \textcolor{red}{1.192} & \textcolor{black}{0.942} & \textcolor{black}{0.937} & \textcolor{black}{0.941} & \textcolor{black}{0.934}\\
oct$(bdshr)$ & \textcolor{red}{1.065} & \textcolor{black}{0.917} & \textcolor{black}{0.909} & \textcolor{black}{0.910} & \textcolor{black}{0.903} & \textcolor{red}{1.084} & \textcolor{black}{0.907} & \textcolor{black}{0.897} & \textcolor{black}{0.898} & \textcolor{black}{0.890}\\
oct$_h(hbshr)$ &  &  &  & \textcolor{black}{0.900} & \textcolor{black}{0.895} &  &  &  & \textcolor{black}{0.883} & \textcolor{black}{0.877}\\
oct$_h(bshr)$ &  &  &  & \textcolor{black}{\textbf{0.876}} & \textcolor{blue}{\textbf{0.871}} &  &  &  & \textcolor{black}{\textbf{0.851}} & \textcolor{blue}{\textbf{0.848}}\\
oct$_h(hshr)$ &  &  &  & \textcolor{black}{0.949} & \textcolor{black}{0.941} &  &  &  & \textcolor{black}{0.945} & \textcolor{black}{0.936}\\
oct$_h(shr)$ &  &  &  & \textcolor{black}{0.890} & \textcolor{black}{0.878} &  &  &  & \textcolor{black}{0.871} & \textcolor{black}{0.858}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 12$}} & \multicolumn{5}{c}{}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.942} & \textcolor{black}{0.947} & \textcolor{black}{0.951} & \textcolor{black}{0.937} &  &  &  &  & \\
ct$(bu)$ & \textcolor{red}{2.990} & \textcolor{black}{0.922} & \textcolor{black}{0.921} & \textcolor{black}{0.923} & \textcolor{black}{0.923} &  &  &  &  & \\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.326} & \textcolor{black}{\textbf{0.779}} & \textcolor{black}{\textbf{0.767}} & \textcolor{black}{0.777} & \textcolor{black}{0.766} &  &  &  &  & \\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.477} & \textcolor{black}{0.804} & \textcolor{black}{0.800} & \textcolor{black}{0.805} & \textcolor{black}{0.799} &  &  &  &  & \\
oct$(ols)$ & \textcolor{black}{\textbf{0.872}} & \textcolor{black}{0.783} & \textcolor{black}{0.784} & \textcolor{black}{0.783} & \textcolor{black}{0.779} &  &  &  &  & \\
oct$(struc)$ & \textcolor{red}{1.077} & \textcolor{black}{0.826} & \textcolor{black}{0.822} & \textcolor{black}{0.823} & \textcolor{black}{0.818} &  &  &  &  & \\
oct$(wlsv)$ & \textcolor{red}{1.149} & \textcolor{black}{0.851} & \textcolor{black}{0.845} & \textcolor{black}{0.847} & \textcolor{black}{0.840} &  &  &  &  & \\
oct$(bdshr)$ & \textcolor{red}{1.021} & \textcolor{black}{0.808} & \textcolor{black}{0.796} & \textcolor{black}{0.796} & \textcolor{black}{0.787} &  &  &  &  & \\
oct$_h(hbshr)$ &  &  &  & \textcolor{black}{0.772} & \textcolor{black}{0.770} &  &  &  &  & \\
oct$_h(bshr)$ &  &  &  & \textcolor{black}{\textbf{0.737}} & \textcolor{blue}{\textbf{0.735}} &  &  &  &  & \\
oct$_h(hshr)$ &  &  &  & \textcolor{black}{0.848} & \textcolor{black}{0.838} &  &  &  &  & \\
oct$_h(shr)$ &  &  &  & \textcolor{black}{0.764} & \textcolor{black}{0.750} &  &  &  &  & \\
\bottomrule
\multicolumn{11}{l}{\rule{0pt}{1em}\rule{0pt}{2em}\textsuperscript{*}\makecell[l]{The Gaussian method employs a sample covariance matrix and includes four techniques (G, B, H, HB)\\ with multi-step residuals.}}\\
\end{tabular}


==> tab/VN525/trash/sam_es_old.tex <==

\begin{tabular}[t]{>{\centering\arraybackslash}p{2.5cm}>{\centering\arraybackslash}p{1.5cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}>{\centering\arraybackslash}p{0.75cm}}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{9}{c}{\textbf{Base forecasts' sample approach}} \\
\cmidrule(l{0pt}r{0pt}){2-10}
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{8}{c}{Gaussian frameworks: sample covariance matrix} \\
\multicolumn{1}{c}{} & \multicolumn{1}{c}{} & \multicolumn{4}{c}{Multi-step residuals} & \multicolumn{4}{c}{\makecell[c]{Overlapping and\\multi-step residuals}} \\
\multirow{-5}{*}{\parbox{2cm}{\centering\textbf{Reconciliation\\approach}}} & \multirow{-4}{*}{Bootstrap} & G & B & H & HB & G & B & H & HB\\
\midrule
\addlinespace[0.3em]
\multicolumn{10}{c}{\textbf{$\forall k \in \{12,6,4,3,2,1\}$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.952} & \textcolor{black}{0.952} & \textcolor{black}{0.954} & \textcolor{black}{0.948} & \textcolor{red}{3.086} & \textcolor{red}{4.372} & \textcolor{black}{0.944} & \textcolor{black}{0.943}\\
ct$(bu_{cs}, bu_{te})$ & \textcolor{red}{2.337} & \textcolor{black}{0.967} & \textcolor{black}{0.966} & \textcolor{black}{0.967} & \textcolor{black}{0.967} & \textcolor{red}{1.020} & \textcolor{red}{1.020} & \textcolor{red}{1.020} & \textcolor{red}{1.020}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.219} & \textcolor{black}{0.871} & \textcolor{black}{0.863} & \textcolor{black}{0.870} & \textcolor{black}{0.863} & \textcolor{black}{0.922} & \textcolor{black}{0.901} & \textcolor{black}{0.922} & \textcolor{black}{0.901}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.318} & \textcolor{black}{0.888} & \textcolor{black}{0.885} & \textcolor{black}{0.889} & \textcolor{black}{0.885} & \textcolor{black}{\textbf{0.882}} & \textcolor{black}{\textbf{0.881}} & \textcolor{black}{0.881} & \textcolor{black}{0.879}\\
oct$(wlsv)$ & \textcolor{red}{1.112} & \textcolor{black}{0.917} & \textcolor{black}{0.913} & \textcolor{black}{0.914} & \textcolor{black}{0.910} & \textcolor{black}{0.908} & \textcolor{red}{24.259} & \textcolor{black}{0.904} & \textcolor{black}{0.902}\\
oct$(bdshr)$ & \textcolor{red}{1.030} & \textcolor{black}{0.888} & \textcolor{black}{0.881} & \textcolor{black}{0.881} & \textcolor{black}{0.875} & \textcolor{black}{0.916} & \textcolor{red}{144.704} & \textcolor{black}{0.884} & \textcolor{black}{0.875}\\
oct$_o(wlsv)$ & \textcolor{red}{1.117} & \textcolor{black}{0.913} & \textcolor{black}{0.910} & \textcolor{black}{0.911} & \textcolor{black}{0.907} & \textcolor{black}{0.904} & \textcolor{red}{22.690} & \textcolor{black}{0.899} & \textcolor{black}{0.896}\\
oct$_o(bdshr)$ & \textcolor{black}{\textbf{0.895}} & \textcolor{black}{\textbf{0.842}} & \textcolor{black}{\textbf{0.822}} & \textcolor{black}{\textbf{0.826}} & \textcolor{blue}{\textbf{0.818}} & \textcolor{red}{2.565} & \textcolor{red}{152.941} & \textcolor{black}{\textbf{0.819}} & \textcolor{black}{\textbf{0.819}}\\
\addlinespace[0.3em]
\multicolumn{10}{c}{\textbf{$k = 1$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.952} & \textcolor{black}{0.950} & \textcolor{black}{0.952} & \textcolor{black}{0.950} & \textcolor{black}{0.944} & \textcolor{black}{0.944} & \textcolor{black}{0.944} & \textcolor{black}{0.943}\\
ct$(bu_{cs}, bu_{te})$ & \textcolor{red}{1.759} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.982} & \textcolor{black}{0.997} & \textcolor{black}{0.998} & \textcolor{black}{0.997} & \textcolor{black}{0.997}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.098} & \textcolor{black}{0.929} & \textcolor{black}{0.928} & \textcolor{black}{0.930} & \textcolor{black}{0.927} & \textcolor{black}{0.944} & \textcolor{black}{0.941} & \textcolor{black}{0.944} & \textcolor{black}{0.941}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.151} & \textcolor{black}{0.940} & \textcolor{black}{0.939} & \textcolor{black}{0.940} & \textcolor{black}{0.938} & \textcolor{black}{\textbf{0.929}} & \textcolor{black}{\textbf{0.928}} & \textcolor{black}{0.929} & \textcolor{black}{0.928}\\
oct$(wlsv)$ & \textcolor{red}{1.050} & \textcolor{black}{0.951} & \textcolor{black}{0.949} & \textcolor{black}{0.950} & \textcolor{black}{0.949} & \textcolor{black}{0.938} & \textcolor{red}{18.299} & \textcolor{black}{0.937} & \textcolor{black}{0.936}\\
oct$(bdshr)$ & \textcolor{red}{1.009} & \textcolor{black}{0.936} & \textcolor{black}{0.933} & \textcolor{black}{0.934} & \textcolor{black}{0.931} & \textcolor{black}{0.936} & \textcolor{red}{106.900} & \textcolor{black}{0.933} & \textcolor{black}{0.930}\\
oct$_o(wlsv)$ & \textcolor{red}{1.052} & \textcolor{black}{0.949} & \textcolor{black}{0.948} & \textcolor{black}{0.948} & \textcolor{black}{0.947} & \textcolor{black}{0.936} & \textcolor{red}{17.061} & \textcolor{black}{0.935} & \textcolor{black}{0.933}\\
oct$_o(bdshr)$ & \textcolor{black}{\textbf{0.950}} & \textcolor{black}{\textbf{0.922}} & \textcolor{black}{\textbf{0.916}} & \textcolor{black}{\textbf{0.918}} & \textcolor{black}{\textbf{0.915}} & \textcolor{red}{2.031} & \textcolor{red}{114.536} & \textcolor{black}{\textbf{0.908}} & \textcolor{blue}{\textbf{0.907}}\\
\addlinespace[0.3em]
\multicolumn{10}{c}{\textbf{$k = 3$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.961} & \textcolor{black}{0.958} & \textcolor{black}{0.960} & \textcolor{black}{0.955} & \textcolor{red}{32.970} & \textcolor{red}{93.338} & \textcolor{black}{0.949} & \textcolor{black}{0.948}\\
ct$(bu_{cs}, bu_{te})$ & \textcolor{red}{2.428} & \textcolor{black}{0.998} & \textcolor{black}{0.997} & \textcolor{black}{0.997} & \textcolor{black}{0.997} & \textcolor{red}{1.041} & \textcolor{red}{1.041} & \textcolor{red}{1.041} & \textcolor{red}{1.042}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.245} & \textcolor{black}{0.911} & \textcolor{black}{0.904} & \textcolor{black}{0.911} & \textcolor{black}{0.904} & \textcolor{black}{0.954} & \textcolor{black}{0.939} & \textcolor{black}{0.953} & \textcolor{black}{0.939}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.348} & \textcolor{black}{0.927} & \textcolor{black}{0.924} & \textcolor{black}{0.928} & \textcolor{black}{0.924} & \textcolor{black}{\textbf{0.916}} & \textcolor{black}{\textbf{0.914}} & \textcolor{black}{0.916} & \textcolor{black}{0.913}\\
oct$(wlsv)$ & \textcolor{red}{1.142} & \textcolor{black}{0.953} & \textcolor{black}{0.949} & \textcolor{black}{0.951} & \textcolor{black}{0.946} & \textcolor{black}{0.939} & \textcolor{red}{25.203} & \textcolor{black}{0.936} & \textcolor{black}{0.933}\\
oct$(bdshr)$ & \textcolor{red}{1.060} & \textcolor{black}{0.926} & \textcolor{black}{0.920} & \textcolor{black}{0.921} & \textcolor{black}{0.915} & \textcolor{black}{0.943} & \textcolor{red}{153.266} & \textcolor{black}{0.924} & \textcolor{black}{0.915}\\
oct$_o(wlsv)$ & \textcolor{red}{1.146} & \textcolor{black}{0.950} & \textcolor{black}{0.947} & \textcolor{black}{0.948} & \textcolor{black}{0.943} & \textcolor{black}{0.933} & \textcolor{red}{23.883} & \textcolor{black}{0.931} & \textcolor{black}{0.928}\\
oct$_o(bdshr)$ & \textcolor{black}{\textbf{0.944}} & \textcolor{black}{\textbf{0.897}} & \textcolor{black}{\textbf{0.878}} & \textcolor{black}{\textbf{0.883}} & \textcolor{black}{\textbf{0.872}} & \textcolor{red}{2.588} & \textcolor{red}{159.608} & \textcolor{black}{\textbf{0.869}} & \textcolor{blue}{\textbf{0.866}}\\
\addlinespace[0.3em]
\multicolumn{10}{c}{\textbf{$k = 12$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{0.942} & \textcolor{black}{0.947} & \textcolor{black}{0.951} & \textcolor{black}{0.937} & \textcolor{black}{0.944} & \textcolor{black}{0.948} & \textcolor{black}{0.940} & \textcolor{black}{0.936}\\
ct$(bu_{cs}, bu_{te})$ & \textcolor{red}{2.990} & \textcolor{black}{0.922} & \textcolor{black}{0.921} & \textcolor{black}{0.923} & \textcolor{black}{0.923} & \textcolor{red}{1.022} & \textcolor{red}{1.023} & \textcolor{red}{1.021} & \textcolor{red}{1.023}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.326} & \textcolor{black}{0.779} & \textcolor{black}{0.767} & \textcolor{black}{0.777} & \textcolor{black}{0.766} & \textcolor{black}{0.871} & \textcolor{black}{0.828} & \textcolor{black}{0.870} & \textcolor{black}{0.828}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.477} & \textcolor{black}{0.804} & \textcolor{black}{0.800} & \textcolor{black}{0.805} & \textcolor{black}{0.799} & \textcolor{black}{\textbf{0.806}} & \textcolor{black}{\textbf{0.807}} & \textcolor{black}{0.805} & \textcolor{black}{0.802}\\
oct$(wlsv)$ & \textcolor{red}{1.149} & \textcolor{black}{0.851} & \textcolor{black}{0.845} & \textcolor{black}{0.847} & \textcolor{black}{0.840} & \textcolor{black}{0.849} & \textcolor{red}{30.955} & \textcolor{black}{0.843} & \textcolor{black}{0.840}\\
oct$(bdshr)$ & \textcolor{red}{1.021} & \textcolor{black}{0.808} & \textcolor{black}{0.796} & \textcolor{black}{0.796} & \textcolor{black}{0.787} & \textcolor{black}{0.870} & \textcolor{red}{184.933} & \textcolor{black}{0.801} & \textcolor{black}{0.787}\\
oct$_o(wlsv)$ & \textcolor{red}{1.156} & \textcolor{black}{0.843} & \textcolor{black}{0.840} & \textcolor{black}{0.841} & \textcolor{black}{0.834} & \textcolor{black}{0.845} & \textcolor{red}{28.669} & \textcolor{black}{0.834} & \textcolor{black}{0.831}\\
oct$_o(bdshr)$ & \textcolor{black}{\textbf{0.800}} & \textcolor{black}{\textbf{0.721}} & \textcolor{black}{\textbf{0.690}} & \textcolor{black}{\textbf{0.695}} & \textcolor{blue}{\textbf{0.687}} & \textcolor{red}{3.208} & \textcolor{red}{195.692} & \textcolor{black}{\textbf{0.696}} & \textcolor{black}{\textbf{0.699}}\\
\bottomrule
\end{tabular}


==> tab/VN525/trash/shr_crps.tex <==

\begin{tabular}[t]{c|>{}cccc>{}c|ccccc}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{10}{c}{\textbf{Base forecasts' sample approach}} \\
\cmidrule(l{0pt}r{0pt}){2-11}
\multicolumn{1}{c}{\makecell[c]{\bfseries Reconciliation\\\bfseries approach}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} \\
\multicolumn{1}{c}{} &  & G & B & H & \multicolumn{1}{c}{HB} &  & G & B & H & HB\\
\midrule
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$\forall k \in \{12,6,4,3,2,1\}$}} & \multicolumn{5}{c}{\textbf{$k = 1$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{\textbf{0.971}} & \textcolor{black}{0.972} & \textcolor{black}{\textbf{0.971}} & \textcolor{black}{0.972} & \textcolor{black}{1.000} & \textcolor{black}{\textbf{0.972}} & \textcolor{black}{0.971} & \textcolor{black}{\textbf{0.972}} & \textcolor{black}{0.971}\\
ct$(bu)$ & \textcolor{red}{1.321} & \textcolor{red}{1.017} & \textcolor{red}{1.018} & \textcolor{red}{1.017} & \textcolor{red}{1.017} & \textcolor{red}{1.077} & \textcolor{black}{0.983} & \textcolor{black}{0.983} & \textcolor{black}{0.983} & \textcolor{black}{0.983}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.057} & \textcolor{red}{1.013} & \textcolor{black}{\textbf{0.971}} & \textcolor{red}{1.013} & \textcolor{black}{0.971} & \textcolor{black}{0.976} & \textcolor{black}{0.987} & \textcolor{black}{\textbf{0.961}} & \textcolor{black}{0.988} & \textcolor{black}{0.961}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.082} & \textcolor{red}{1.020} & \textcolor{black}{0.978} & \textcolor{red}{1.020} & \textcolor{black}{0.978} & \textcolor{black}{0.986} & \textcolor{black}{0.991} & \textcolor{black}{0.964} & \textcolor{black}{0.991} & \textcolor{black}{0.964}\\
oct$(wlsv)$ & \textcolor{black}{0.987} & \textcolor{red}{1.080} & \textcolor{red}{1.041} & \textcolor{black}{0.992} & \textcolor{black}{0.958} & \textcolor{black}{0.952} & \textcolor{red}{1.004} & \textcolor{black}{0.969} & \textcolor{black}{0.978} & \textcolor{black}{0.956}\\
oct$(bdshr)$ & \textcolor{black}{\textbf{0.975}} & \textcolor{red}{1.072} & \textcolor{red}{1.032} & \textcolor{black}{0.985} & \textcolor{blue}{\textbf{0.950}} & \textcolor{blue}{\textbf{0.949}} & \textcolor{black}{0.999} & \textcolor{black}{0.965} & \textcolor{black}{0.975} & \textcolor{black}{\textbf{0.952}}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 2$}} & \multicolumn{5}{c}{\textbf{$k = 3$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{\textbf{0.969}} & \textcolor{black}{0.969} & \textcolor{black}{\textbf{0.968}} & \textcolor{black}{0.968} & \textcolor{black}{1.000} & \textcolor{black}{\textbf{0.971}} & \textcolor{black}{\textbf{0.970}} & \textcolor{black}{\textbf{0.969}} & \textcolor{black}{0.970}\\
ct$(bu)$ & \textcolor{red}{1.189} & \textcolor{black}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.000} & \textcolor{red}{1.273} & \textcolor{red}{1.013} & \textcolor{red}{1.013} & \textcolor{red}{1.013} & \textcolor{red}{1.013}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.015} & \textcolor{red}{1.004} & \textcolor{black}{\textbf{0.968}} & \textcolor{red}{1.004} & \textcolor{black}{0.968} & \textcolor{red}{1.041} & \textcolor{red}{1.013} & \textcolor{black}{0.973} & \textcolor{red}{1.014} & \textcolor{black}{0.973}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.031} & \textcolor{red}{1.009} & \textcolor{black}{0.973} & \textcolor{red}{1.009} & \textcolor{black}{0.973} & \textcolor{red}{1.062} & \textcolor{red}{1.020} & \textcolor{black}{0.979} & \textcolor{red}{1.020} & \textcolor{black}{0.979}\\
oct$(wlsv)$ & \textcolor{black}{0.972} & \textcolor{red}{1.064} & \textcolor{red}{1.021} & \textcolor{black}{0.987} & \textcolor{black}{0.958} & \textcolor{black}{0.983} & \textcolor{red}{1.083} & \textcolor{red}{1.041} & \textcolor{black}{0.993} & \textcolor{black}{0.960}\\
oct$(bdshr)$ & \textcolor{black}{\textbf{0.964}} & \textcolor{red}{1.057} & \textcolor{red}{1.015} & \textcolor{black}{0.983} & \textcolor{blue}{\textbf{0.953}} & \textcolor{black}{\textbf{0.972}} & \textcolor{red}{1.075} & \textcolor{red}{1.033} & \textcolor{black}{0.988} & \textcolor{blue}{\textbf{0.955}}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 4$}} & \multicolumn{5}{c}{\textbf{$k = 6$}}\\
base & \textcolor{black}{1.000} & \textcolor{black}{\textbf{0.973}} & \textcolor{black}{\textbf{0.973}} & \textcolor{black}{\textbf{0.971}} & \textcolor{black}{0.973} & \textcolor{black}{1.000} & \textcolor{black}{\textbf{0.976}} & \textcolor{black}{0.977} & \textcolor{black}{\textbf{0.975}} & \textcolor{black}{0.977}\\
ct$(bu)$ & \textcolor{red}{1.340} & \textcolor{red}{1.021} & \textcolor{red}{1.021} & \textcolor{red}{1.021} & \textcolor{red}{1.021} & \textcolor{red}{1.450} & \textcolor{red}{1.032} & \textcolor{red}{1.033} & \textcolor{red}{1.032} & \textcolor{red}{1.033}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.061} & \textcolor{red}{1.018} & \textcolor{black}{0.974} & \textcolor{red}{1.018} & \textcolor{black}{0.974} & \textcolor{red}{1.094} & \textcolor{red}{1.023} & \textcolor{black}{\textbf{0.974}} & \textcolor{red}{1.024} & \textcolor{black}{0.974}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.087} & \textcolor{red}{1.025} & \textcolor{black}{0.981} & \textcolor{red}{1.026} & \textcolor{black}{0.981} & \textcolor{red}{1.127} & \textcolor{red}{1.033} & \textcolor{black}{0.984} & \textcolor{red}{1.033} & \textcolor{black}{0.984}\\
oct$(wlsv)$ & \textcolor{black}{0.990} & \textcolor{red}{1.100} & \textcolor{red}{1.059} & \textcolor{black}{0.996} & \textcolor{black}{0.959} & \textcolor{red}{1.001} & \textcolor{red}{1.115} & \textcolor{red}{1.076} & \textcolor{black}{0.998} & \textcolor{black}{0.958}\\
oct$(bdshr)$ & \textcolor{black}{\textbf{0.977}} & \textcolor{red}{1.091} & \textcolor{red}{1.049} & \textcolor{black}{0.989} & \textcolor{blue}{\textbf{0.952}} & \textcolor{black}{\textbf{0.985}} & \textcolor{red}{1.103} & \textcolor{red}{1.064} & \textcolor{black}{0.989} & \textcolor{blue}{\textbf{0.949}}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 12$}} & \multicolumn{5}{c}{}\\
base & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{\textbf{0.968}} & \textcolor{black}{\textbf{0.969}} & \textcolor{black}{\textbf{0.969}} & \textcolor{black}{0.971} &  &  &  &  & \\
ct$(bu)$ & \textcolor{red}{1.675} & \textcolor{red}{1.056} & \textcolor{red}{1.057} & \textcolor{red}{1.057} & \textcolor{red}{1.057} &  &  &  &  & \\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.163} & \textcolor{red}{1.032} & \textcolor{black}{0.974} & \textcolor{red}{1.033} & \textcolor{black}{0.974} &  &  &  &  & \\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.212} & \textcolor{red}{1.043} & \textcolor{black}{0.987} & \textcolor{red}{1.044} & \textcolor{black}{0.987} &  &  &  &  & \\
oct$(wlsv)$ & \textcolor{red}{1.025} & \textcolor{red}{1.122} & \textcolor{red}{1.085} & \textcolor{red}{1.001} & \textcolor{black}{0.954} &  &  &  &  & \\
oct$(bdshr)$ & \textcolor{red}{1.002} & \textcolor{red}{1.110} & \textcolor{red}{1.071} & \textcolor{black}{0.989} & \textcolor{blue}{\textbf{0.941}} &  &  &  &  & \\
\bottomrule
\multicolumn{11}{l}{\rule{0pt}{1em}\rule{0pt}{2em}\textsuperscript{*}\makecell[l]{The Gaussian method employs a shrinkage covariance matrix and includes four techniques (G, B, H, HB)\\ with multi-step residuals.}}\\
\end{tabular}


==> tab/VN525/trash/shr_es.tex <==

\begin{tabular}[t]{c|>{}cccc>{}c|ccccc}
\toprule
\multicolumn{1}{c}{\textbf{}} & \multicolumn{10}{c}{\textbf{Base forecasts' sample approach}} \\
\cmidrule(l{0pt}r{0pt}){2-11}
\multicolumn{1}{c}{\makecell[c]{\bfseries Reconciliation\\\bfseries approach}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} & \multicolumn{1}{c}{ctjb} & \multicolumn{4}{c}{\makecell[c]{Gaussian approach\textsuperscript{*}}} \\
\multicolumn{1}{c}{} &  & G & B & H & \multicolumn{1}{c}{HB} &  & G & B & H & HB\\
\midrule
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$\forall k \in \{12,6,4,3,2,1\}$}} & \multicolumn{5}{c}{\textbf{$k = 1$}}\\
base & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{\textbf{0.958}} & \textcolor{black}{0.984} & \textcolor{black}{\textbf{0.972}} & \textcolor{black}{0.992} & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{\textbf{0.954}} & \textcolor{black}{0.958} & \textcolor{black}{\textbf{0.954}} & \textcolor{black}{0.958}\\
ct$(bu)$ & \textcolor{red}{2.427} & \textcolor{red}{1.040} & \textcolor{red}{1.042} & \textcolor{red}{1.040} & \textcolor{red}{1.041} & \textcolor{red}{1.759} & \textcolor{red}{1.001} & \textcolor{red}{1.002} & \textcolor{red}{1.002} & \textcolor{red}{1.002}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.243} & \textcolor{black}{0.988} & \textcolor{black}{\textbf{0.913}} & \textcolor{black}{0.990} & \textcolor{blue}{\textbf{0.913}} & \textcolor{red}{1.098} & \textcolor{red}{1.011} & \textcolor{black}{\textbf{0.938}} & \textcolor{red}{1.013} & \textcolor{blue}{\textbf{0.938}}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.348} & \textcolor{red}{1.020} & \textcolor{black}{0.940} & \textcolor{red}{1.022} & \textcolor{black}{0.939} & \textcolor{red}{1.151} & \textcolor{red}{1.028} & \textcolor{black}{0.950} & \textcolor{red}{1.030} & \textcolor{black}{0.950}\\
oct$(wlsv)$ & \textcolor{red}{1.132} & \textcolor{red}{1.137} & \textcolor{red}{1.065} & \textcolor{red}{1.059} & \textcolor{black}{0.969} & \textcolor{red}{1.050} & \textcolor{red}{1.078} & \textcolor{black}{0.989} & \textcolor{red}{1.043} & \textcolor{black}{0.960}\\
oct$(bdshr)$ & \textcolor{red}{1.047} & \textcolor{red}{1.085} & \textcolor{red}{1.013} & \textcolor{red}{1.011} & \textcolor{black}{0.927} & \textcolor{red}{1.009} & \textcolor{red}{1.050} & \textcolor{black}{0.966} & \textcolor{red}{1.019} & \textcolor{black}{0.942}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 2$}} & \multicolumn{5}{c}{\textbf{$k = 3$}}\\
base & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{\textbf{0.960}} & \textcolor{black}{0.971} & \textcolor{black}{\textbf{0.958}} & \textcolor{black}{0.972} & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{\textbf{0.963}} & \textcolor{black}{0.981} & \textcolor{black}{\textbf{0.966}} & \textcolor{black}{0.986}\\
ct$(bu)$ & \textcolor{red}{2.176} & \textcolor{red}{1.035} & \textcolor{red}{1.036} & \textcolor{red}{1.035} & \textcolor{red}{1.035} & \textcolor{red}{2.428} & \textcolor{red}{1.042} & \textcolor{red}{1.044} & \textcolor{red}{1.042} & \textcolor{red}{1.043}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.192} & \textcolor{red}{1.020} & \textcolor{black}{\textbf{0.942}} & \textcolor{red}{1.021} & \textcolor{blue}{\textbf{0.942}} & \textcolor{red}{1.245} & \textcolor{red}{1.009} & \textcolor{black}{\textbf{0.931}} & \textcolor{red}{1.011} & \textcolor{blue}{\textbf{0.931}}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.275} & \textcolor{red}{1.045} & \textcolor{black}{0.962} & \textcolor{red}{1.047} & \textcolor{black}{0.962} & \textcolor{red}{1.348} & \textcolor{red}{1.038} & \textcolor{black}{0.955} & \textcolor{red}{1.040} & \textcolor{black}{0.954}\\
oct$(wlsv)$ & \textcolor{red}{1.110} & \textcolor{red}{1.149} & \textcolor{red}{1.065} & \textcolor{red}{1.070} & \textcolor{black}{0.979} & \textcolor{red}{1.142} & \textcolor{red}{1.160} & \textcolor{red}{1.082} & \textcolor{red}{1.073} & \textcolor{black}{0.981}\\
oct$(bdshr)$ & \textcolor{red}{1.045} & \textcolor{red}{1.105} & \textcolor{red}{1.024} & \textcolor{red}{1.033} & \textcolor{black}{0.949} & \textcolor{red}{1.060} & \textcolor{red}{1.109} & \textcolor{red}{1.032} & \textcolor{red}{1.029} & \textcolor{black}{0.943}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 4$}} & \multicolumn{5}{c}{\textbf{$k = 6$}}\\
base & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{\textbf{0.962}} & \textcolor{black}{0.987} & \textcolor{black}{\textbf{0.973}} & \textcolor{black}{0.996} & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{\textbf{0.963}} & \textcolor{black}{0.998} & \textcolor{black}{\textbf{0.984}} & \textcolor{red}{1.011}\\
ct$(bu)$ & \textcolor{red}{2.585} & \textcolor{red}{1.052} & \textcolor{red}{1.054} & \textcolor{red}{1.053} & \textcolor{red}{1.053} & \textcolor{red}{2.849} & \textcolor{red}{1.083} & \textcolor{red}{1.085} & \textcolor{red}{1.083} & \textcolor{red}{1.084}\\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.277} & \textcolor{red}{1.000} & \textcolor{blue}{\textbf{0.923}} & \textcolor{red}{1.002} & \textcolor{black}{\textbf{0.923}} & \textcolor{red}{1.339} & \textcolor{black}{0.999} & \textcolor{black}{\textbf{0.921}} & \textcolor{red}{1.000} & \textcolor{blue}{\textbf{0.920}}\\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.392} & \textcolor{red}{1.032} & \textcolor{black}{0.950} & \textcolor{red}{1.035} & \textcolor{black}{0.950} & \textcolor{red}{1.473} & \textcolor{red}{1.038} & \textcolor{black}{0.954} & \textcolor{red}{1.040} & \textcolor{black}{0.954}\\
oct$(wlsv)$ & \textcolor{red}{1.157} & \textcolor{red}{1.167} & \textcolor{red}{1.097} & \textcolor{red}{1.075} & \textcolor{black}{0.982} & \textcolor{red}{1.192} & \textcolor{red}{1.187} & \textcolor{red}{1.124} & \textcolor{red}{1.090} & \textcolor{black}{0.995}\\
oct$(bdshr)$ & \textcolor{red}{1.065} & \textcolor{red}{1.112} & \textcolor{red}{1.041} & \textcolor{red}{1.025} & \textcolor{black}{0.939} & \textcolor{red}{1.084} & \textcolor{red}{1.121} & \textcolor{red}{1.058} & \textcolor{red}{1.029} & \textcolor{black}{0.940}\\
\addlinespace[0.3em]
\multicolumn{1}{c}{} & \multicolumn{5}{c}{\textbf{$k = 12$}} & \multicolumn{5}{c}{}\\
base & \textcolor{black}{\textbf{1.000}} & \textcolor{black}{0.948} & \textcolor{red}{1.010} & \textcolor{red}{1.002} & \textcolor{red}{1.033} &  &  &  &  & \\
ct$(bu)$ & \textcolor{red}{2.990} & \textcolor{red}{1.028} & \textcolor{red}{1.031} & \textcolor{red}{1.029} & \textcolor{red}{1.029} &  &  &  &  & \\
ct$(shr_{cs}, bu_{te})$ & \textcolor{red}{1.326} & \textcolor{black}{\textbf{0.897}} & \textcolor{black}{\textbf{0.830}} & \textcolor{black}{\textbf{0.899}} & \textcolor{blue}{\textbf{0.830}} &  &  &  &  & \\
ct$(wls_{cs}, bu_{te})$ & \textcolor{red}{1.477} & \textcolor{black}{0.942} & \textcolor{black}{0.872} & \textcolor{black}{0.945} & \textcolor{black}{0.870} &  &  &  &  & \\
oct$(wlsv)$ & \textcolor{red}{1.149} & \textcolor{red}{1.089} & \textcolor{red}{1.041} & \textcolor{red}{1.006} & \textcolor{black}{0.922} &  &  &  &  & \\
oct$(bdshr)$ & \textcolor{red}{1.021} & \textcolor{red}{1.015} & \textcolor{black}{0.964} & \textcolor{black}{0.935} & \textcolor{black}{0.855} &  &  &  &  & \\
\bottomrule
\multicolumn{11}{l}{\rule{0pt}{1em}\rule{0pt}{2em}\textsuperscript{*}\makecell[l]{The Gaussian method employs a shrinkage covariance matrix and includes four techniques (G, B, H, HB)\\ with multi-step residuals.}}\\
\end{tabular}

